Unsupervised Few-Shot Action Recognition via Action-Appearance Aligned Meta-Adaptation

We present MetaUVFS as the first Unsupervised Meta-learning algorithm for Video Few-Shot action recognition. MetaUVFS leverages over 550K unlabeled videos to train a two-stream 2D and 3D CNN architecture via contrastive learning to capture the appearance-specific spatial and action-specific spatio-temporal video features respectively. MetaUVFS comprises a novel Action-Appearance Aligned Meta-adaptation (A3M) module that learns to focus on the action-oriented video features in relation to the appearance features via explicit few-shot episodic meta-learning over unsupervised hard-mined episodes. Our action-appearance alignment and explicit few-shot learner conditions the unsupervised training to mimic the downstream few-shot task, enabling MetaUVFS to significantly outperform all unsupervised methods on few-shot benchmarks. Moreover, unlike previous few-shot action recognition methods that are supervised, MetaUVFS needs neither base-class labels nor a supervised pretrained backbone. Thus, we need to train MetaUVFS just once to perform competitively or sometimes even outperform state-of-the-art supervised methods on popular HMDB51, UCF101, and Kinetics100 few-shot datasets.

==> sections/experiments_copy.tex <==
\section{Experiments and Results}
% This section describes our experimental setup: training and evaluation details, followed by results, analysis  and observations.
\input{tables/external_meta_uvfs}
% \input{tables/FSVAR_SS+ablations}
\subsection{Datasets} 
We evaluate \methodname~on three publicly-available few-shot datasets: Kinetics100 \cite{carreira2019short, zhu2018compound}, UCF101 \cite{soomro2012ucf101} and HMDB51 \cite{kuehne2011hmdb}. Following~\cite{zhu2018compound}, we obtain the \textit{few-shot}  train/validation/test splits with 64/12/24 non-overlapping classes for Kinetics100. For UCF101 and HMDB51, we follow the \textit{few-shot} split from \cite{zhang2020few}. UCF101 contains 100 classes split into 70/10/20 and HMDB51 contains 51 classes split as 31/10/10. The test splits of each dataset are used for novel class evaluation in the meta-testing phase. For the unsupervised training of \methodname's two-stream networks, we leverage Kinetics700~\cite{carreira2019short} without using any labels. Kinetics700 is a large-scale video classification dataset that covers 700 human action classes including human-object and human-human interactions. To increase the size of our unlabeled training data, we also include the videos from the base-classes of Kinetics100, UCF101, and HMDB51, without the labels. Altogether, we obtain around $550$K video clips with a duration of around 10s each (25 FPS). We take extra precaution to ensure that there is no video in the training dataset belonging to the union of all the novel classes across all three evaluation datasets. This is to ensure that our testing is truly on a disjoint set of unseen classes.               

\subsection{Implementation Details}
\noindent{\bf Data Sampling and Augmentation}
\label{sec:sampling}
We develop a spatio-temporal sampling protocol that is most optimal for the unsupervised two-stream training and A3M-based few-shot training/testing. For an input video, the 2D appearance stream encodes 8 input frames where 1 frame is randomly sampled from each of 8 segments equally-partitioned along the video length. With focus on spatial information, we use a higher frame resolution of $224 \times 224$. We refer to this as $8\times1$.  For the 3D-action stream, with the goal of encoding fine-grained spatio-temporal action information across video segments, we sample 4 clips across 4 equidistant segments of the video to form a 16 frame input. To balance the spatio-temporal information, we use a lower frame resolution of $112 \times 112$. We refer to this as $4\times4$. 
% in the interest of scaling of  contrastive training on  larger batch size and time-efficiency for full-training on our large dataset.  
We follow SimCLR's protocol for spatial augmentation~\cite{chen2020simple}: a composition of Random crops, Random horizontal flips, Random Color Jitter, Random grayscale, Gaussian blur. The spatial augmentation is clip-wise consistent, \ie, the random seed is fixed across all frames of a video augmentation~\cite{xu2019self,han2020memory}.  
% At a spatial-level, our data augmentation  follows SimCLR \cite{chen2020simple}: a composition of Random crops, Random horizontal flips, Random Color Jitter, Random grayscale, Gaussian blur. These augmentations are applied on the input clip level: randomness is fixed for all frames in the video. Random sampling of frames (appearance) or clips (action) within video segments, provide temporal augmentations.
\paragraph{MetaUVFS Training} 
We use ResNet50~\cite{he2016deep} backbone to train the 2D appearance stream and its 3D counterpart, ResNet50-3D~\cite{hara3dcnns}, for the 3D action stream. The dimension of $z^{ap}$ and $z^{act}$ obtained from the MLP projection head is 128~(similar to~\cite{chen2020simple}).
% For an unlabeled video $x_i$, the input to the 2D appearance network contain 8 frames that are fed sequentially and to obtain 8 2048-dimensional feature encodings. These 8 features are averaged to obtain the single encoding $h^{ap}_i$. The input video clip to the 3D action encoder network consists of 16 frames from the $4 \times 4$ sampling which is encoded into a 2048-dimensional feature encoding $h^{act}_i$. These encodings, $h^{ap}_i$ and $h^{act}_i$,   defined in Section~\ref{sec:twostream} are fed to MLP projection heads to obtain 128-dimension feature encodings $z^{ap}$ and $z^{act}$ respectively (similar to~\cite{chen2020simple}).
 We first train the action and appearance streams individually using losses $\mathcal{L}^{ap}_{NCE}$ and $\mathcal{L}^{act}_{NCE}$ respectively. We use a batch size of 512 and train both models for 300 epochs on 64 NVIDIA P100 GPUs. Following~\cite{he2019bag, goyal2017accurate}, we do a gradual learning rate (LR) warmup for 5 epochs followed by a half-period cosine learning rate decay with SGD optimizer and 0.9 momentum. With 0.001 per-gpu LR, we also linearly scale the LR to 0.064. 
%  We use SGD as the optimizer with a momentum of 0.9.

For hard-mining episodes, $n$ is set to 32. We set $d_k=128$ and $d_v=2048$ for the A3M module. For MAML, we set $E=10$, $\alpha=0.001$ and $\beta=10$. We train for $20,000$ iterations using Adam optimizer and cosine annealing~\cite{antoniou2018train} for a total of $200K$ unsupervised hard-mined episodes. For more details, please refer to the supplementary material.
%  A3M  the query and key linear maps of each transformer share weights \cite{doersch2020crosstransformers} and each have dimensions $q_{dim}$=$k_{dim}$=128. To train MAML, inner loop LR is 10 and epochs is 10 while outer loop is LR is 0.001 and number of episodes 10000. For more details, please refer to the supplementary material.
 
\paragraph{Few-shot Evaluation} We evaluate \methodname~on all three datasets based on 5-way, 1-shot and 5-way, 5-shot settings as is standard in few-shot learning literature.
% Standard protocol in few-shot learning literature is followed to evaluate \methodname~on 5-way, 1-shot and 5-way, 5-shot settings. 
For each episode, 5 classes are randomly sampled from the set of novel classes for classification and training happens on 1 and 5 support samples per class respectively. In all settings, Top-1 accuracy is reported on 1 query sample per class. 
% We test in both settings on all three datasets. 
In each experiment, we randomly sample 10,000 episodes for few-shot meta-testing and report the average accuracy and the 95\% confidence interval. Finetuning is done at a constant learning rate of 10 for 50 epochs for all experiments.

\input{tables/ablation_meta_uvfs}
\subsection{Compare to SoTA Unsupervised Approaches}
Table~\ref{tab:fsvar} compares \methodname~with various state-of-the-art supervised and unsupervised methods on different few-shot settings and datasets. We categorize the different techniques based on the amount of supervision in terms of base-class data (`Yes' in \textit{Base-Class}) and surrogate supervision, \ie, initializing the network using the weights pretrained on a large-scale supervised image/video data (`Yes' in \textit{Pretrained Weights}). Cells are left blank if there are no publicly available results for that setting. 

The second part of Table~\ref{tab:fsvar} compares \methodname~with various state-of-the-art methods that leverage unlabeled videos for representation learning. To the best of our knowledge, \methodname~is the first approach that specializes in few-shot action recognition in a purely unsupervised manner. Hence, there is no publicly available benchmark for the performance of existing video-based unsupervised techniques on few-shot action recognition. We took the initiative to assess these approaches on our few-shot test-bed using the same hyperparameters for few-shot meta-testing as \methodname. Many of these approaches are originally trained on a relatively small unlabeled dataset. Therefore, for a fair comparison, we train these methods on our large-scale unlabeled dataset using their publicly available code.
% and utilizing the hyper-parameters from each paper on the same unlabeled training datasets of ours. 
% We could not include PRP \cite{yao2020video} that is originally trained on UCF101 as we could not reproduce it on our large dataset due to NaN issues. 

% The second part of Table~\ref{tab:fsvar} summarizes the results of our comparison on few-shot benchmarks with existing unsupervised video methods. 
As shown in Table~\ref{tab:fsvar}, \methodname~is able to clearly outperform all state-of-the-art unsupervised methods on the task of few-shot action recognition by at least 13.38\%, 3.34\% and 9.54\% (absolute increase) on UCF101, HMDB51 and Kinetics100 1-shot, 5-way benchmark respectively. Among the methods we compare, IIC~\cite{tao2020self}, CVRL~\cite{qian2020spatiotemporal} and CoCLR~(RGB only)~\cite{Han20CoCLR} also use contrastive loss for unsupervised training. The superior performance of \methodname~in comparison to these methods indicate that our approach of jointly leveraging and aligning action and appearance along with meta-training episodically for few-shot plays an integral role in performing effectively when the downstream task lies in the low-shot regime.

\subsection{Compare to SoTA Supervised Few-shot Works}
The first part of Table~\ref{tab:fsvar} compares \methodname~with various state-of-the-art supervised few-shot action recognition methods.
% for few-shot action recognition on different few-shot settings and datasets. We categorize and group the different techniques based on the amount of supervision in terms of base-class data (`Yes' in \textit{Base Class}) and surrogate supervision, \ie, initializing the network using the weights pretrained on a large-scale supervised image/video data (`Yes' in \textit{Pretrained Weights}). Cells are left blank if there are no publicly available results for that setting. 
We can observe that compared to ARN~\cite{zhang2020few} that uses only base-class data as supervision, \methodname~significantly outperforms on UCF101 and HMDB51, and performs competitively on Kinetics100. Furthermore, \methodname~is even able to outperform some of the supervised methods that use both pretrained weights and base-class labels for supervision such as ProtoGAN~\cite{kumar2019protogan} on UCF101 and HMDB51, and CMN~\cite{zhu2018compound} on Kinetics100. It is worth noting that, unlike these methods that need to train separate models to obtain results on the different datasets, \methodname~trains a \textit{single} unsupervised model to achieve all results. This single model either outperforms or performs competitively compared to supervised methods across all three datasets.

% \subsection{Compare to SoTA Supervised Few-shot Methods}
% Table~\ref{tab:fsvar} compares \methodname~with various state-of-the-art methods for few-shot action recognition on different few-shot settings and datasets. We categorize and group the different techniques based on the amount of supervision in terms of base-class data (`Yes' in \textit{Base Class}) and surrogate supervision, \ie, initializing the network using the weights pretrained on a large-scale supervised image/video data (`Yes' in \textit{Pretrained Weights}). Cells are left blank if there are no publicly available results for that setting. We can observe that compared to ARN~\cite{zhang2020few} that uses only base-class data as supervision, \methodname~significantly outperforms on UCF101 and HMDB51, and performs competitively on Kinetics100. Furthermore, \methodname~is even able to outperform some of the supervised methods that use both pretrained weights and base-class labels for supervision such as ProtoGAN~\cite{kumar2019protogan} on UCF101 and HMDB51, and CMN~\cite{zhu2018compound} on Kinetics100. It is worth noting that unlike these methods that need to train separate models to obtain results on the different datasets, \methodname~trains a single unsupervised model to achieve all results. This single model is able to either outperform or perform competitively compared to supervised methods across all three datasets.

% \subsection{Compare to SoTA Unsupervised Approaches}
% We compare \methodname~with various state-of-the-art methods that leverage unlabeled videos for representation learning. To the best of our knowledge, \methodname~is the first approach that specializes for few-shot action recognition in a purely unsupervised manner. Hence, there is no publicly available benchmark for the performance of existing video-based unsupervised techniques on few-shot action recognition. We took the initiative to assess these approaches on our few-shot testbed using the same hyperparameters for few-shot meta-testing as \methodname. Many of these approaches are originally trained on a relatively small unlabeled dataset. Therefore, for a fair comparison, we train these methods on our large-scale unlabeled dataset using their publicly available code.
% % and utilizing the hyper-parameters from each paper on the same unlabeled training datasets of ours. 
% % We could not include PRP \cite{yao2020video} that is originally trained on UCF101 as we could not reproduce it on our large dataset due to NaN issues. 

% % The second part of Table~\ref{tab:fsvar} summarizes the results of our comparison on few-shot benchmarks with existing unsupervised video methods. 
% As shown in second part of Table~\ref{tab:fsvar}, \methodname~is able to clearly outperform all state-of-the-art unsupervised methods on the task of few-shot action recognition by at least 13.38\%, 3.34\% and 9.54\% (absolute increase) on UCF101, HMDB51 and Kinetics100 1-shot, 5-way benchmark respectively. Among the methods we compare, IIC~\cite{tao2020self}, CVRL~\cite{qian2020spatiotemporal} and CoCLR~\cite{Han20CoCLR} also use contrastive loss for unsupervised training. The superior performance of \methodname~in comparison to these methods indicate that our approach of jointly leveraging and aligning action and appearance along with meta-training episodically for few-shot plays an integral role in performing effectively when the downstream task lies in the low-shot regime.


% jointly leveraging multiple streams in terms of action and appearance plays an integral role in performing effectively when the downstream task lies in the low-data regime. 

\subsection{\methodname: Ablation Study}
We conduct an ablation study where we isolate individual aspects of \methodname~and quantify their impact on the few-shot performance. Table~\ref{tab:ablation} summarizes the results. We train all ablation experiments using MAML as the few-shot algorithm. We first conduct experiments where the network consists of either action or appearance stream but not both (Table~\ref{tab:ablation}, Row 1-2). We directly feed the features from the available stream (averaging appearance features over 8 frames) to the classifier layer for few-shot episodic meta-training and later for meta-testing. A3M module is not present in these two experiments as it is not compatible when both streams are not present for alignment.  For a fair comparison and to also delineate the impact of the A3M module and action-appearance stream, we also do an experiment where both action and appearance stream are present. There we simply concatenate the action features and appearance features (averaged over 8 frames) and feed to the classifier for few-shot episodic meta-training without A3M. All three experiments use unsupervised hard-mined episodes. In the absence of a stream, only the features of the available stream are used to mine episodes. 

We can observe from Table~\ref{tab:ablation}~(Row 1,~2,~4) that the few-shot performance is significantly worse when either action or appearance stream is missing compared to when both are present as proposed by our method. This is because when only a few support samples are available to learn for a set of novel classes, the likelihood of the model to make mistakes reduces sharply in the presence of both streams as it allows the network more ways to activate and respond to the representative features necessary for correct classification. Row 4 and 6 highlight the impact of aligning action-appearance via A3M as part of few-shot training. Our proposed A3M module in MetaUVFS results in an average absolute improvement of 3.22\% and 1.47\% on 5-way, 1-shot and 5-shot benchmark across all datasets. Aligning the action and appearance features during few-shot episodic training significantly improves the model’s ability to \textit{attend} to the most representative video aspects while leveraging the inductive biases of both 2D and 3D CNNs to learn complementary representation that boosts few-shot performance. We can also compare Row 1~(Action only) with CVRL~\cite{qian2020spatiotemporal} in Table~\ref{tab:fsvar}. CVRL backbone is similar to our 3D action stream. However, due to an explicit few-shot training phase, our \textit{Action only}' baseline performs consistently better than CVRL. 

We also perform an experiment where we train our method episodically without mining hard episodes based on noise-contrastive embeddings to highlight its importance. We can observe from Row 4-6 that there is a significant reduction in performance without hard episodes making mining hard episodes crucial to the few-shot episodic training of \methodname. This is because in the absence of hard episodes, the randomly sampled videos in a training episode are such that the action and appearance embeddings fed for support and query augmentation samples to A3M during training are already highly separable. This severely impedes the training of A3M and makes it behave close to an identity function, as is also evident from its only slightly improved performance than Row 4 where A3M is not present at all. 

We also perform an experiment where both A3M and hard episodes are absent during training (Table~\ref{tab:ablation}, Row 3). We can observe that this setting results in a statistically significant reduction in performance compared to when  A3M and/or hard episodes are present (Row 4-6).

% \subsection{\methodname: Ablation Study}
% To highlight the impact of individual aspects of \methodname~ on its few-shot performance, we conduct an ablation study where we isolate these  aspects and test the few-shot performance on 5-way, 1-shot and 5-way, 5-shot setting on Kinetics100. Table~\ref{tab:ablation} summarizes the results.

% Table~\ref{tab:ablation} first shows the performance of using either only the appearance stream or the action stream in \methodname. We observe that in both scenarios, the few-shot performance is significantly worse than those achieved by leveraging both action and appearance streams. The intuition is when only a few support samples are available to learn about data belonging to novel classes, the likelihood of the model making mistakes reduces sharply in the presence of both streams as it allows the network more ways to activate and respond to the representative features necessary for correct classification. The third row of Table~\ref{tab:ablation} shows when we only maximize the mutual information between views within the two streams but do not jointly maximize the mutual information between the two streams. We observe that this also reduces the few-shot performance, highlighting the effect of MM-NCE loss on the few-shot performance by jointly optimizing multiple streams and facilitating the learning of more generalizable video representations.



\input{tables/sampling}
\subsection{Discussion}
\label{sec:discussion}
{\noindent \bf Impact of Frame Sampling.} Since the two-streams in \methodname~specialize both in terms of architecture and their function, we observe that the sampling strategy in choosing the frames as input to both streams along with their frame resolution make a difference in the performance. Table~\ref{tab:Sampling} provides an analysis of the few-shot performance for 5-way, 1-shot settings on Kinetics100 across different sampling strategies for both 3D action and 2D appearance streams first individually and then in combination. We observe that for the 3D stream, choosing a $4 \times 4$ sampling, \ie, sampling 4 segments of 4 frames uniformly over the entire video length provides a $3.3\%$ improvement over sampling 16 frames from 32 consecutive frames with a stride of 2. Similarly, for the 2D stream, we find that $16 \times 1$ and $8 \times 1$ sampling, \ie, sampling 1 frame from 16 or 8 segments over the entire video length as  most effective. In our two-stream setting, we find $8 \times 1$, $4 \times 4$ as the optimal sampling scheme. 
% Through experimentation, we find that choosing the right frame sampling makes a significant difference in performance. In Table~\ref{tab:Sampling} we can see that for 3D Stream, frame sampling of 32-16 to 4x4 is a 5\% increase in the 1shot task. The 2D stream, we find that the 4x1 frame capture is more effective in capturing long-term spatial features. 
% \begin{figure}
% \begin{center}
%   \includegraphics[width=\columnwidth]{sections/figures/lr_plot_log.pdf}
% \end{center}
%   \caption{Performance vs Steps for Kinetics 100 1 shot/5 way}
% \label{fig:lr_plot}
% \end{figure}

% \begin{figure}
% \begin{center}
%   \includegraphics[width=\columnwidth]{sections/figures/many_way_plot.pdf}
% \end{center}
%   \caption{Performance vs Steps for Kinetics 100 1 shot/5 way}
% \label{fig:many_way}
% \end{figure}
\begin{figure}
\begin{center}
  \includegraphics[width=\columnwidth]{sections/figures/many_way_metauvfs.pdf}
\end{center}
\vspace{-1em}
  \caption{
%   (a) Comparison of accuracy for 1-shot, 5-way task on Kinetics100 for finetuning with different learning rate and number of steps. (b) 
  Comparison of \methodname~ with CVRL~\cite{qian2020spatiotemporal} on UCF101 and Kinetics100 dataset on 1-shot few-shot for N-way classification where N ranges from 5 to over 20.}
\label{fig:many_way}
\vspace{-1em}
\end{figure}

\input{tables/ablation_meta_learning}
{\noindent \bf Meta-learning Algorithm.} We further validate the choice of MAML as our few-shot meta-learning algorithm by assessing other popular few-shot approaches in the literature. To compare with ProtoNet~\cite{snell2017prototypical} and ProtoMAML~\cite{triantafillou2019meta}, we repurpose the output of A3M module to compute prototypes across support samples (augmentations) and compare against query samples to compute the loss during training. For few-shot testing on novel classes, ProtoNet matches the query samples with prototypes that are computed from support samples to assign class label based on the best matched prototype. For ProtoMAML, we reshape the prototypes computed from support samples as parameters of the classifier layer which is finetuned along with the A3M module as per Sec.~\ref{sec:fs_testing}. We also compare with Baseline++~\cite{chen2018closer} where we use meta-trained parameters for A3M and classifier but change the few-shot finetuning during testing to Baseline++. As shown in Table~\ref{tab:meta_learning}, we find that our few-shot meta-testing protocol of using MAML with $l_2$-normalized embedding as input to the classifier significantly outperforms other few-shot learning methods. We also observe that, in general, few-shot methods employing finetuning during few-shot testing tend to perform better. We believe this is due to extra adaptation steps needed during testing because of the absence of supervision during training. 
% {\noindent \bf Meta-learning Algorithm.} We further validate the choice of a transfer learning approach for few-shot meta-testing by assessing other popular meta-testing approaches in the literature. Given our self-supervised meta-training setting in \methodname, we find it suitable to compare our finetuning strategy with ProtoNets ~\cite{snell2017prototypical} and Baseline++ ~\cite{chen2019closer} with results provided in Table~\ref{tab:fsvar}. Our transfer-learning based few-shot evaluation is significantly better than ProtoNet which we believe is because ProtoNet requires an episodic `meta-training' phase using base class supervision to function optimally, the lack of which causes the performance reduction. Although Baseline++ is close to our few-shot setup, from empirical results, it does not perform as well as finetuning.
%%%%%%%%%%%% move to supplementary %%%%%%%%%%%%%%%%%%
% {\noindent \bf Learning rate.} As our few-shot meta-testing is formulated as a transfer learning approach, we observe that the learning rate and the number of steps to train the classifier on support samples are fundamental to achieving the optimal performance. Figure~\ref{fig:many_way} provides insights into the effect of different learning rates and number of steps to fine-tune have on the few-shot performance. Note that since we use $l_2$-normalized representation as the input to the classifier, higher learning rates such as 1 or 10 can be used for faster convergence. However, very high learning rates such as 100 can lead to overfitting and reduced performance.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%In our experiments with evaluating the performance of \methodname~ on the few-shot benchmarks following a transfer learning approach, we observed that learning rate and the steps to finetune the classifier played crucial role in achieving the optimal performance. Table~\ref{tab:LRtable} provides insights into the effect of different learning rates and number of steps to fine tune plays on the few-shot performance.



% Comparing ProtoNet \cite{snell2017prototypical} vs Cosine distance classifier and Simple Finetuning \cite{chen2019closer}. Gaurav talk's about results here refering to the table.


% \paragraph{Impact of pretraining} In the interest of providing a complete analysis on our few-shot settings, we also test the performance of training a classifier over features obtained from publicly available pretrained backbones. Table~\ref{tab:fsvar} provides results for these experiments. We observe that in some scenarios the performance of these backbones can be higher than $95\%$ on our few-shot settings. In these scenarios, we believe that there is a high likelihood of the existence of an overlap between the training data used to train these backbones and the novel classes we use for testing as these backbones and corresponding training datasets are not designed from the few-shot benchmark perspective.  

% \paragraph{Few-shot Nearest Neighbor Retrieval} To better understand the working of our method, we perform a qualitative study wherein we use the support samples to retrieve nearest neighbors from the set of novel class video samples. Figure [] depicts the results of this experiment. [include some failure cases as well]

% \input{tables/mixed_data}
%{\noindent \bf Many-way Few Shot.} We go beyond the 5-way 1-shot setting by increasing the number of novel classes to 10, 15 and 21/24 to evaluate SeSuMI on the more challenging general many-way classification problem. Fig.~\ref{fig:many_way} shows a plot for the few-shot performance on UCF101 and Kinetics100 as we increase the N in 1-shot, N-way classification task. As expected, the performance reduces with increasing N. However, compared to CVRL~\cite{qian2020spatiotemporal}, \methodname~is able to maintain a significant margin and with the gap in performance widening a bit for UCF101 and remaining the same for Kinetics100. This highlights the robustness of our learnt representations in classifying videos with 1-shot training example when the number of novel classes increase.


%We also show results where we increase the number of classes in any given episode to more than 5 and perform few-shot experiments to demonstrate the effectiveness of our approach in a practical few-shot scenario.
\input{tables/ablation_action_appearance}
{\noindent \bf Significance of Action-Appearance} We conduct an experiment where both the streams are either 3D CNNs~(action) or 2D CNNs~(appearance).  This delineates the impact of having complementary action and appearance streams on few-shot performance from the impact of increase in the parameter count due to an additional backbone. We train them using MAML with hard episodes without A3M for fair comparison. We can observe from Table~\ref{table:aa} that although having more parameters with either two appearance or two action streams improves the performance compared to single stream, the improvement is significantly higher when a combination of action and appearance streams is used that helps to leverage more diverse 2D/3D representations to learn more generalizable few-shot video representations.  

{\noindent \bf Many-Way Few Shot.} We go beyond the 5-way 1-shot setting by increasing the number of novel classes 
% to 10, 15 and 21/24 
to evaluate \methodname~on a more challenging and \textit{in-the-wild} few-shot many-way classification task on UCF101 and Kinetics100. Fig.~\ref{fig:many_way} shows a plot for this experiment. Although, as expected, the performance reduces with increasing N, \methodname~is still able to outperform the best-performing unsupervised baseline method, CVRL, by a significant margin for all N-way 1-shot classification tasks considered.
% compared to CVRL~\cite{qian2020spatiotemporal}, \methodname~is able to maintain a significant margin and with the gap in performance widening a bit for UCF101 and remaining the same for Kinetics100. 
% This highlights the effectiveness of \methodname~that has an explicit few-shot meta-learner in classifying videos with 1-shot training example when any number of novel classes.
% This further proves the effectiveness of using action-appearance aligned features and performing explicit few-shot meta-training for a downstream few-shot task.
This proves that \methodname~is more robust even in extreme few-shot scenarios where the inter-class confusion is higher. 
% We believe our work will encourage future efforts to leverage larger-scale unlabeled video data.
% \paragraph{Mixed domain few shot} 

% As noted before, we train a single unified model in our method on a large-scaled unlabeled dataset using self-supervision and test across all few-shot settings using this model. Consequently, our approach is not confined to the distribution of any given dataset and has the potential to generalize on classes across a diverse set of datasets. To demonstrate this, we conduct an experiment where we pool the novel class data from all the three datasets we consider and randomly sample 10K episodes where in each episode, each of the randomly sampled classes can belong to any of the datasets. Table~\ref{tab:mixed} summarizes the results of this experiment. 


% \subsection{Adding some supervision}

==> sections/intro_bkp.tex <==
\section{Introduction}
%Over the past decade, deep learning has been instrumental in achieving superior performance on tasks spanning over a broad industrial spectrum. However, their ability to provide strong performance across datasets is restricted by the availability of large-scale clean, labeled and task-specific data that is needed to train high capacity models that can generalize well. Obtaining labeled data, especially for every different tasks, is often expensive and intractable to scale. Consequently, few-shot learning \cite{koch2015siamese, sung2018learning,
% vinyals2016matching,
% gidaris2018dynamic,
% snell2017prototypical,
% ravi2016optimization,
% koch2015siamese,
% finn2017model,
% chen2019closer,
% hariharan2017low,
% wang2018low} has emerged as a class of techniques that aim to solve the problem of lack of large-scale supervision by training the model to quickly learn to generalize to unseen data samples using as low as a single reference sample.


Growth of visual multi-media consumption has presents a strong need for deep learning models that learn to generalize over wide variety of datasets. However, training such high capacity models to generalize across diverse datasets required labeled data which  at-scale can be impractical due to labor costs or domain  knowledge requirements for wildlife, medical imaging etc datasets. . Few-shot learning \cite{koch2015siamese, sung2018learning,
vinyals2016matching,
gidaris2018dynamic,
snell2017prototypical,
ravi2016optimization,
koch2015siamese,
finn2017model,
chen2019closer,
hariharan2017low,
wang2018low} are a class of techniques which aim to solve this problem by learning models that can quickly recognize unseen data samples with as low as one or five training samples. 


With annotation a lot more scarcer in video data, few-shot learning can prove to be an effective solution in learning highly efficient video representations. However,  few-shot learning in videos are relatively less explored as videos have a temporal dimension in addition to spatial. Prior works in this domain have designed specialized modules on top of 2D CNN's \cite{zhu2018compound,Cao_2020_CVPR, fu2020depth} and recently 3D models \cite{xian2020generalized,cao2020few, zhang2020few} have report stronger results keeping the same 'meta-testing' evaluaton protocol. Nevertheless, the overfitting in training video models persists as the limited base class videos might not be sufficient parameter-heavy networks. To address this issue, augmenting input RGB  video clips with depth \cite{fu2020depth}
or auxiliary self-supervision losses \cite{zhang2020few} have been explored however labelled base class supervision is required to be competitive on video few-shot benchmarks. In addition to base class supervision, most of these methods initialize their models on supervised image or video pretrained weights which proves to be a strong prior on the overall performance. Since base class labels comprise a majority ratio in these few-shot datasets, we believe that it restricts the existing methods to perform cross-domain or generalize across diverse new datasets. Therefore in our work, we try to answer the question: \textit{"Can we develop models that perform competitive on few-shot benchmarks without the use of base class labels?"}

\begin{figure}[t]
\begin{center}
%\fbox{\rule{0pt}{2in} \rule{0.9\linewidth}{0pt}}
   \includegraphics[width=\linewidth]{sections/figures/teaser.png}
\end{center}
   \caption{Appearance-stream and Action-Stream[Placeholder image]}
\label{fig:teaser}
\end{figure}

Acquiring unlabelled data to learn diverse and robust representations via self-supervision can be a cheaper alternative that can be finetuned on varied downstream applications mostly commonly being classification \cite{noroozi2016unsupervised, zhang2016colorful, gidaris2018unsupervised, doersch2015unsupervised, he2020momentum}. Methods using contrastive learning have been most effective thus far to leverage large-scale unlabelled data \cite{he2020momentum, chen2020simple}. Here the task defines each input sample in a large training batch to be its own class optimizes the network learns to identify high-level spatial semantics to match and discriminate heavily augmented versions of the a given input sample with other samples. 



Two-stream pathways captures feature specific to scene(long-term dynamics) and short term dynamics action dynamics. Similar two-stream slowfast and simple feature aggregation like video recognition techniques. During meta-testing we just finetune. 
Inspired by these works, we that adapts the contrastive loss objective to compare augmented pair of video clips from the same unlabelled video to learn spatio spatio-temporal video representations. In Fig~\ref{fig:teaser}

Apart from multi-stream network design, we also show that shows qualitative and quantitative performance that proves our method being better suited to few shot video recognition as compared to concurrent approaches similar to ours for generic video representation learning \cite{qian2020spatiotemporal, Han20CoCLR}. 

% Why our self supervised learning using two steam and 3stream refer here to the teaser diagram to explain how our unsupervised method is most effective for few shot task.  The better the
% self-supervision, the better the downstream performance. Large-scale weakly-supervised pre-training for video action recognition \cite{ghadiyaram2019large}

%  Recognizing actions such
% as “opening the door” requires careful modeling of temporal ordering. In the video classification literature, 3D convolution and optical flow are two main-stream methods to
% model short-term temporal relations [38, 41], while longterm temporal relations are usually neglected.
% There is growing interest in learning models capable of
% effectively adapting themselves to recognize novel classes
% with only a few training examples. This is known as fewshot learning [10, 14]. Meta-learning is a promising approach for few-shot learning, the model is explicitly trained to deal with scarce training data for different episodes [12]. While the majority
% of recent few-shot learning work focuses on image classification, its extension to video classification is not trivial.
%  State-of-theart approaches commonly apply a temporal pooling module
% (usually mean pooling) in order to make final predictions
% [22, 41]. As observed in [47], averaging the deep features
% only captures the co-occurrence rather than the temporal or10618 1
% dering of patterns, which inevitably result in information
% loss.
% Nevertheless, most few-shot classification methods still require much annotated data for pre-training.
% Recently, several unsupervised meta-learning approaches, constructing episodes via pseudo-labeling
% (Hsu et al., 2019; Ji et al., 2019) or image augmentations (Khodadadeh et al., 2019; Antoniou and
% Storkey, 2019; Qin et al., 2020), have addressed this problem. To our knowledge, unsupervised
% non-episodical techniques for transfer learning to few-shot tasks have not yet been explored.

To summarize our contributions, 
\begin{enumerate}
    \item  We propose to leverage  large-scale unlabelled video data (550K) using self-supervision to learn a single model whose feature representations are generalizable  and adapt quickly to novel classes in few-shot setting.
    \item  We propose \methodname, a novel video two-stream model that maximizes the mutual information across  spatial-focused 2D network and spatio-temporal 3D network through a contrastive based novel loss called MMCELoss.
    \item To the best of our knowledge, we are the first to demonstrate results for Unsupervised Video Few Shot Learning on publicly available action recognition datasets and provide a strong benchmark for future research. 
    \item Our method significantly outperforms \textit{state-of-the-art} supervised few-shot video recognition methods and self-supervised video representation learning methods.
      

\end{enumerate}

==> sections/intro_bkp_mar_15.tex <==

\section{Introduction}
Few-shot learning \cite{koch2015siamese, sung2018learning,
vinyals2016matching,
gidaris2018dynamic,
snell2017prototypical,
ravi2016optimization,
koch2015siamese,
finn2017model,
chen2019closer,
hariharan2017low,
wang2018low} has emerged as a school of approaches that aim to tackle the problem of lack of large-scale supervision by training the model to quickly learn to generalize to unseen data using as few as a single labeled data point. It is highly relevant for videos which have a temporal dimension in addition to spatial that makes the task more complex and harder to annotate. Prior work have utilized both 2D CNNs~\cite{zhu2018compound,Cao_2020_CVPR, fu2020depth} and 3D CNNs~\cite{xian2020generalized,cao2020few, zhang2020few} to achieve strong results on few-shot action recognition. 

% Over the last decade, supervised approaches employing deep neural networks have achieved superior performance on a broad spectrum of tasks. However, their ability to generalize, i.e. to achieve the same strong performance across different datasets, can be limited due to the lack of large-scale, well distributed, clean labeled data. Obtaining large quantities of quality labeled data is often difficult and expensive. Consequently, few-shot learning \cite{koch2015siamese, sung2018learning,
% vinyals2016matching,
% gidaris2018dynamic,
% snell2017prototypical,
% ravi2016optimization,
% koch2015siamese,
% finn2017model,
% chen2019closer,
% hariharan2017low,
% wang2018low} has emerged as a school of approaches that aim to tackle the problem of lack of large-scale supervision by training the model to quickly learn to generalize to unseen data using as few as a single labeled data point.

\begin{figure}[t]
\begin{center}
  \includegraphics[width=\linewidth]{sections/figures/teaser_muvfs.pdf}
\end{center}
   \caption{Above, we consider a 2D CNN (appearance), 3D CNN (action)  and ours \methodname~ trained on the same unlabeled dataset and fine-tuned on a 1-support 5-way task.  For the query video of \textit{Tennis Swing}, the 2D CNN relies on  frame-level spatial cues and incorrectly relates a person standing on a green-orange background with \textit{Jump Rope} having a similar background. The 3D action CNN  captures the swinging action of the query video however inaccurately labels it with \textit{Golf Swing} that has similar spatio-temporal  characteristics as \textit{Tennis Swing} support. \methodname's A3M module finds the alignment over these two-stream features -- appearance on action, thus predicting the correct class.}
\label{fig:teaser}
\end{figure}

All these methods follow the standard few-shot learning protocol where there is a set of \textit{base} classes with relatively large number of labeled samples and a set of \textit{novel} classes with samples that are unseen to the model. The \textit{base} class data is used to train the model in a \textit{meta-training} phase to learn to classify using as few reference samples as possible. The model is then evaluated in a \textit{meta-testing} phase where it classifies samples~(query) from a subset of the novel classes based on few (typically one or five) labeled examples~(support). This way of supervised few-shot learning is limited by the amount of base-class data in its ability to generalize to novel classes from highly diverse domains \cite{doersch2020crosstransformers}. 

Although there are approaches that mitigate this by relying on large-scale supervised pretraining~\cite{Cao_2020_CVPR, cao2020few, fu2020depth, xian2020generalized}, large-scale supervision is prohibitively expensive to scale and often times unattainable. Howevev, there is virtually infinite amount of unlabeled video data at our disposal thanks to multi-media social networking. This motivates us to answer the question, \textit{``Can we develop models for action recognition that perform competitively on few-shot benchmarks without the use of either base class labels or any external supervision?’’}


% Few-shot learning in videos is relatively less explored as videos have a temporal dimension in addition to spatial making the task more complex. Prior work in this domain have designed specialized modules on top of 2D CNNs \cite{zhu2018compound,Cao_2020_CVPR, fu2020depth}  while more recent approaches employ three dimensional (3D) models \cite{xian2020generalized,cao2020few, zhang2020few} to achieve stronger results. These methods follow the standard few-shot learning protocol where there is a set of `base’ classes for which relatively large number of labeled samples are available, and there is a set of `novel’ classes whose samples are unseen to the model. The `base’ class data is used to train the model to learn to classify using as few reference samples as possible in what is termed the `meta-training’ phase. The model is then evaluated in a `meta-testing' phase where it classifies samples from a subset of the novel classes based on few (typically one or five) support examples. These methods are limited by the size of the base class dataset in their ability to generalize to novel classes from highly diverse domains \cite{doersch2020crosstransformers}. To address this over-fitting issue, some approaches have explored augmenting input RGB video clips with depth \cite{fu2020depth} or auxiliary self-supervision losses \cite{zhang2020few}; some introduce surrogate supervision by initializing the models weights using  pre-trained backbones on large-scale supervised image/video classification tasks ~\cite{Cao_2020_CVPR, cao2020few, fu2020depth, xian2020generalized}. Although supervised pre-training helps, it is prohibitively expensive to scale and often times unattainable. 

%------ new text added here onwards----%

% Although large-scale labeled videos are not always available, there is virtually infinite amount of unlabeled video data at our disposal thanks to multi-media social networking. This motivates us to answer the question, \textit{``Can we develop models for action recognition that perform competitively on few-shot benchmarks without the use of either base class labels or any external supervision?’’}

Access to unlabeled data has led to a growing interest in unsupervised feature representation learning in  vision~\cite{grill2020bootstrap, he2020momentum}  and language~\cite{devlin2018bert, brown2020language} tasks. Amongst these, methods employing contrastive learning~(InfoNCE)~\cite{oord2018representation} have been the most effective in harnessing large-scale unlabeled  data ~\cite{he2020momentum, chen2020simple, qian2020spatiotemporal}, where their performance in  vision tasks has been comparable to supervised methods.  These methods assume that testing phase will have same classes it was finetuned on.  Moreover, the full-size labeled dataset requirements for transfer learning on downstream task is crucial difference to few-shot settings where the distinct separation in novel-base class data distribution. Previous supervised \cite{finn2017model,ravi2016optimization} and unsupervised \cite{khodadadeh2019unsupervised, khodadadeh2019unsupervised, hsu2018unsupervised} meta-learning literature show that features learned with task-based training that can learn to quickly adapt to a novel classes during testing using only few labeled samples.  

Building upon these insights, we propose the first method \methodname~, for Unsupervised video Few shot Action Recognition. MetaUVFS in meta-training, learns unsupervised video representations via contrastive learning from a large unlabelled dataset. Later, it trains an explicit few-shot meta-learner by generating unlabelled episodes that mined from the  learnt video representations. By imposing a task-specific prior on learnt video representations  through episodic learning in the meta-training phase, it mimics the settings in the meta-test phase there-by reduce the knowledge gap between training and testing. MetaUVFS outperforms or performs competitively to the state-of-the-art (SoTA) few-shot action recognition methods and outperforms all unsupervised video learning methods on multiple benchmark datasets. 

We introduce a two-stream network to learn fine-grained spatio-temporal features over video segments through action stream, the spatial features that are consistent through the video are encoded via an appearance stream. Direct finetuning of each of these feature stream in a challenging few-shot scenarios illustrated in Fig.~\ref{fig:teaser} can be sub-optimal. Instead, we propose to learn spatio-temporal alignment of appearance over action features to obtain salient  features shared by samples of the same class (intra-class) and alleviates confusion that is inter-class. This Action-Appearance Alignment is parameterized through an unsupervised Meta-adaptation phase (A3M) where unlabelled tasks are generated from the two-stream deep features.  Thus the objective of A3M is four-folds, 1) generate unlabeled tasks by mining hard instances from unsupervised features, 2) learn a meta-learner that learns cross-alignment in the outer-loop, and 3) rapidly learn to classify unlabeled tasks in the inner-loop. 4. During meta-testing,  A3M is prepared for few-shot classification receiving novel class support-query features from the two-stream network. Overall, \methodname~'s design comprising of  two-stream networks and the A3M module are highly optimized for video few-shot  application and empirically yields a wide gap between a conventional approach of direct fine-tuning.


%%%%%%% older version %%%%%%%
% Although large scale labeled videos are not always available, there is virtually infinite amount of unlabeled video data at our disposal thanks to multi-media social networking. This motivates the growing interest in unsupervised approaches for robust feature representation learning in  vision~\cite{grill2020bootstrap, he2020momentum}  and language~\cite{devlin2018bert, brown2020language} tasks. Amongst these, the ones that employ contrastive learning~(InfoNCE)~\cite{oord2018representation} have been the most effective in large-scale datasets. ~\cite{he2020momentum, chen2020simple, qian2020spatiotemporal}. In this work, we try to answer the question, \textit{``Can we develop models for action recognition that perform competitively on few-shot benchmarks without the use of either base class labels or any external supervision?’’}


% In our work, we propose an Unsupervised Video Few-Shot method (\methodname) to learn video representation using self-supervision, to perform unsupervised meta-learning such that it acquires priors on the downstream few-shot learning task to compete or outperform methods that use supervision. Our method comprises of a two-stream action and appearance network that learns unsupervised video representations and a dedicated attentive meta-adaptation module that functions as a few-shot classifier during training and test phases. 

% We find that efficient video representations can be learned by processing the ‘action’ and ‘appearance’ associated with a video both independently and jointly rather than simply using a 3D convolutional network, observation in-line with earlier work [13, 51]. (\methodname) comprises of a two-stream path-
% way to capture the frame-level `appearance' using a 2D CNN
% and fine-grained actions across video segments using a 3D CNN. Stream representations learned independently by leveraging a large-scale unlabelled dataset (550k samples) using contrastive learning.  

% In challenging few-shot scenarios illustrated in Fig. 1, the spatio-temporal alignment of appearance over action stream enhances salient features that is intra-class and alleviates confusion that is inter-class. To that end, we introduce Attentive Meta-Adaptation (AMA) module that parametrizes this cross alignment via meta-learning. Additionally, it imposes a task-specific prior on input two-stream features by introducing tasks in the training phase that mimics the settings in the test phase to reduce the gap between training and test settings. Thus the objective of AMA is three-fold: generate unlabelled tasks by mining hard instances from unsupervised features  2. learn a meta-learner that learns cross-alignment in the outer-loop 3. and rapid learns unlabelled tasks in the inner-loop. During meta-testing,  AMA functions as a dedicated few-shot classifier receiving novel class support-query features from the two-stream network. To conclude, our  AMA module with action-appearance networks are highly optimized for few-shot video application and empirically, this design yields a wide gap between a straightforward approach of directly finetuning these representations on novel classes.  


To summarize, our main contributions are as follows,

\begin{enumerate}
\item We propose \methodname, to solve a challenging problem of unsupervised few-shot action recognition.

\item \methodname~ design comprises two-stream network to learn action and appearance-specific features using self-supervision. An A3M module  generates meta-learning episodes by tasks from from two-stream features and their parametrizes their alignment. During meta-testing, A3M is effective as a dedicated fews-shot classifier. 
\item We successfully demonstrate that task-specific unsupervised representations can be mined from over a half a million (550K) unlabeled videos. For practical use, \methodname~ can be a highly effective proxy to supervised pre-training, which to best of our knowledge, is the first work in this domain. 
\item  \methodname~ performs competitively or even outperforms some of the    SoTA (all supervised) few-shot action recognition methods across multiple benchmarks. Its also shown empirically,  that SoTA video self-supervised methods by design are not effective in few-shot regime.
\end{enumerate}

% In contrastive learning, the network is trained to correctly match each input sample with an augmented version of itself among a large training batch of other samples and their respective augmented selves. 
% Our model  provides the best way to leverage use of large unlabelled data which is lacking in design in previous methods. 
% goal of mining positive samples by using
% other complementary views of the data. A lot of tasks are trivial so learning in meta-learning phase may collapse. To be clear, we are not proposing a new loss function or pretext task here, but instead we target the
% training regime by improving the sampling process in the contrastive learning of visual representation,
% i.e. constructing positive pairs beyond instances. There is another aspect that base-class may suffer from overfitting from training on base class going to novel classes. Our first contribution is to explore using self-supervision to overcome supervision collapse. \cite{doersch2020crosstransformers}


% 1. two-stream design why? why not directly finetuning?  why hard negative mining? why attention  why not joint optimization, ? why maml?
%  multiple representation streams of video data samples via a novel MM-NCE loss.
 
%  To begin addressing these problems, we propose an unsupervised meta-learning method: one which
% aims to learn a learning procedure, without supervision, that is useful for solving a wide range of
% new, human-specified tasks. With only raw, unlabeled observations, our model’s goal is to learn
% a useful prior such that, after meta-training, when presented with a modestly-sized dataset for a
% human-specified task, the model can transfer its prior experience to efficiently learn to perform the
% new task. To perform unsupervised meta-learning, we need to automatically construct tasks from unlabeled
% data.
% In our work, we employ contrastive learning as an effective tool to leverage large-scale unlabelled video dataset and there are several differences with recent methods. First, we learn general purpose features using an RGB-only two-stream approach that effectively aligns spatial and spatial-temporal cues in a cross-attention framework. Secondly, these features are optimized for few-shot performance: we apply unsupervised meta-adaption on hardest tasks mined from the unlabelled data. % use in methods \cite{chen2020simple, he2020momentum} ours is   we restrict our approach to RGB inputs as computing optical flow can be resource-intensive and has scalability issues especially with a large-scale dataset as ours having $\sim$550K videos. 

% \item SeSuMI is not confined within the distribution of any given dataset. This single model is more practical and can accommodate in-the-wild few shot scenarios where the classes are from a mixed data distribution.


==> sections/method_bkp.tex <==
\section{Method}
%\methodname~ aims to learn feature representations over unlabeled videos that are highly generalizable/adaptable and can learn to classify videos from a disjoint novel set of classes with few labeled samples~(shots). It is designed to capture the different salient aspects of a video in terms of temporal action and visual appearance separately and simultaneously by leveraging a two-stream network that is trained end-to-end in a self-supervised manner. To the best of our knowledge, this is also the first effort to train such an end-to-end two-stream network for large-scale video-based self-supervision. Section [] describes the network design for our method. Inspired by the most recent developments in self-supervised learning [cite], we design a novel multi-view multi-stream formulation of the InfoNCE loss, termed as MM-NCE loss, that is tailored specifically to maximize mutual information among the different views and different modalities of the underlying unlabeled video data. Section [] provides an overview of the optimization procedure. Finally, we describe our approach to perform few shot learning on novel set of video classes using the self-supervised trained model.

The goal of \methodname~is to learn feature representations over unlabeled videos that are highly generalizable/adaptable and can learn to classify videos from a disjoint novel set of classes with few labeled samples~(shots). To this end, \methodname ~employs a two-stream architecture that learns to represent the information related to the action and appearance of the video separately and simultaneously. The network is trained end-to-end in a self-supervised manner using a novel multi-view multi-stream contrastive loss, termed as MM-NCE loss. To the best of our knowledge, \methodname~is the first effort to train an end-to-end two stream network for large-scale video-based self-supervision. Figure~\ref{fig:sesumi_model} provides a detailed illustration of \methodname. The following subsections describe our method.

% In this section, we introduce our VideoCLR for few-shot video classification . Our approach in Figure 1 consists of 1) a representation learning 
% stage which trains a 2D and 3D model on the large unlabelled base class dataset. 2. We learn a joint representation by maximizing the mutual information across these two networks. 3. We perform an episodic training using a linear classifier on the l2 normed network encodings on novel classes with few labeled videos, and 4) a
% testing stage which evaluates the model on unseen test videos. The details of each of these stages are given below.
\subsection{Two-stream architecture}
% Figure [] depicts the network architecture of \methodname. We posit that in order to learn highly generalizable feature representations over videos for the task of action recognition, it is essential for the network to capture the visual information of the scene independently and also in correlation with the temporal dynamics in the video. To this end, we design a two-stream feedforward architecture that operates on the RGB information of the video. The \textit{appearance stream} employs 2D convolutional filters to learn spatial feature maps over the different frames of the video and treat the frames independent of each other, whereas the \textit{action stream} employs 3D convolutional filters to learn spatio-temporal feature maps jointly over one or more frames~(the collection of which we term as video segment). 

% Informed by [cite feature pyramid related papers], we argue that it is important to perform hierarchical feature aggregation by pooling the features learned at different resolutions in the two streams. Therefore, every time we downsample the features in each of the streams, we perform a global average pooling across height, width and time dimensions and concatenate the features with the output of the backbone.

We posit that in order to learn highly generalizable feature representations over videos for the task of few-shot action recognition, it is essential for the network to capture the visual information of the scene independently and also in correlation with the temporal dynamics in the video. To this end, we design a two-stream feedforward architecture that operates on the RGB information of the video. 

On one hand, we have the \textit{appearance stream} that employs 2D CNN to learn spatial feature maps over the different frames of the video. The frames are sampled over a longer time horizon and the corresponding feature maps are averaged to output an embedding $h^{ap}_i$  that captures the high-level visual semantics over the entire video. On the other hand, we have the \textit{action stream} that employs 3D convolutional filters to learn spatio-temporal feature maps jointly over multiple video clip segments. The embedding $h^{act}_i$ obtained from the \textit{action stream} captures the spatio-temporal semantics within the different video segments.

\subsection{Multi-view Multi-modal Noise Contrastive Estimation (MM-NCE)}
 %SeSuMI only has access to unlabeled video data. It faces an unsupervised representation learning problem where the objective is to learn a function $g$ that maps the unlabeled data into a lower-dimensional space where the target few-shot action recognition task can be performed effectively. We leverage the InfoMax principle [] in doing so and aim to learn $g$ such that it maximizes the mutual information~(MI) between input $x$ and its representation $z$. Inspired by recent approaches [], we adopt a multi-view formulation of the InfoMax objective as it enables us to maximize mutual information directly between the low-dimensional learned representations of the multiple views of the original unlabeled data $X$ such that the views can span different modalities and aspects (in terms of spatio-temporal augmentations). 
 
 With access to only unlabeled video data, the objective of \methodname~is to learn a function $g$ that maps the unlabeled data into a lower-dimensional space where the target few-shot action recognition task can be performed effectively. We leverage the InfoMax principle~\cite{linsker1988self} for this and model $g$ such that it maximizes the mutual information~(MI) between input $x$ and its representation $z = g(x)$. Inspired by recent approaches~\cite{oord2018representation, tian2019contrastive}, we adopt a multi-view formulation of the InfoMax objective as it enables us to maximize mutual information directly between the low-dimensional learned representations of the multiple views of the original unlabeled data $x$ where views can span different modalities and spatio-temporal augmentations.

The multi-view MI formulation is as follows. Given a video $x$, let $x_i$ and $x_j$ be two \textit{views} of $x$. Let $g_1$ and $g_2$ be the encoders that generate representations $g_1(x_i)$ and $g_2(x_j)$ respectively. The objective for unsupervised feature representation learning is to maximize the mutual information between the representations of the two views as follows,
\begin{equation}
    \max_{g_1 \in \mathcal{G}_2, g_2 \in \mathcal{G}_2} I \left( g_1(x_i);g_2(x_j) \right)
\end{equation}
where $I(x_i;x_j)$ is the MI estimator. In our work, we use InfoNCE~\cite{oord2018representation} as the MI estimator defined as,
\begin{equation}
    I(x_i;x_j) \geq \mathbb{E} \left[ \frac{1}{K} \sum_{i=1}^K \log \frac{e^{f(x_i, y_i)}}{\frac{1}{K}\sum_{j=1}^K e^{f(x_i, y_i)}} \right] \triangleq I_{NCE} (X;Y)
\end{equation}
[details related to above equation, projection head etc]
Based on experiments, we choose to adopt the SimCLR~\cite{chen2020simple} version of InfoNCE loss, called NT-Xent loss, where the contrastive loss between a pair of positive samples $i,j$ is given as, 
\begin{equation}
    l^{\text{NT-Xent}} (x_i, x_j) = - \log \frac{e^{sim(\mathbf{z}_i, \mathbf{z}_j)/\tau}}{\sum_{k=1}^{2N} \mathbbm{1}_{[k\neq i]} e^{sim(\mathbf{z}_i, \mathbf{z}_k)/\tau}}
\end{equation}
where sim$(.,.)$ is the cosine similarity between $\mathbf{z}_i$ and $\mathbf{z}_j$ and $\tau$ is a temperature scalar.

The vanilla NT-Xent loss maximizes the agreement between two augmented views of the same input data sample where just one encoder is used to generate representations for both views. Since \methodname~ employs a two-stream architecture to learn more generalizable feature representations from the unlabeled video data, we propose a novel variant of the NT-Xent loss, called \textit{MM-NCE loss}, to better adapt to videos, described in the following paragraphs. %and our network design consisting of two separate encoders. The different aspects of MM-NCE loss are described in following paragraphs.


\subsection{Data Sampling and Augmentation}
For our multi-view multi-stream contrastive learning formulation, we place high emphasis on the sampling and augmentation strategies being critical to few-shot performance. As illustrated in Fig~\ref{fig:teaser} given a video input, the 2D appearance stream encodes an 8 frames input sequentially, where 1 frame is randomly sampled across 8 equal segments along the video length. Since there is more focus on the spatial visual information we consider a higher resolution~$(224 \times 224)$. We refer this as 8x1.  On the other hand, for the 3D-action stream, the goal is to encode fine-grained spatio-temporal action information across video segments. Therefore, we sample 4 clips across 4 segments of the video frames to form a 16 frame input. Here we take the frame resolution~$(112 \times 112)$ because  it allows contrastive training on larger batch size, 2. time-efficiency for full-training on our large dataset 3. negligible performance change in few-shot task. 

Our data augmentation policy follows SimCLR \cite{chen2020simple}: a composition of Random crops, Random horizontal flips, Random Color Jitter, Random grayscale, Gaussian blur. These augmentations are applied on input clip level: randomness is fixed for all frames in the video. Augmentation on temporal level consists of  the frames or clips being sampled randomly within  video segments.


\paragraph{Action and Appearance Multi-stream Contrastive Learning} We randomly sample a mini-batch of $N$ videos where for each video $x_i$, we generate four (instead of two) augmnetations that serve as four views of $x_i$. Two of these augmentations are propagated through the \textit{appearance stream} of SeSuMI generating embeddings $h^{ap}_{2k-1}$ and $h^{ap}_{2k}$. These representations are then transformed into $z^{ap}_{2k-1}$ and $z^{ap}_{2k}$ respectively with a non-linear multilayer perceptron (MLP) projection head. We then apply the contrastive loss, $\mathcal{L}^{ap}_{NCE}$ between all pairs of positive examples with respect to all possible pairs of samples propagated through the 2D appearance stream. We take the other two augmentations and propagate them through the \textit{action stream} of SeSuMI. The resulting embeddings $h^{act}_{2k-1}$ and $h^{act}_{2k}$ are then transformed into $z^{act}_{2k-1}$ and $z^{act}_{2k}$ via another non-linear MLP projection head and the final embeddings are subjected to the contrastive loss, $\mathcal{L}^{act}_{NCE}$, similar to the 2D appearance stream.

%\paragraph{Joint Contrastive Loss} The embeddings, $h^{ap}_{2k}$ and $h^{act}_{2k}$, obtained from the 2D and 3D encoder streams respectively help us to separately encode the visual information of the video independently and also jointly with the temporal information of the video. However, as we mentioned earlier, the learned video representations need to encode both simultaneously in order to generalize well to novel classes with few labeled samples. We therefore introduce a third non-linear MLP projection head that takes the concatenation of $h^{ap}_{2k}$ and $h^{act}_{2k}$ as input to output $z^{joint}_{2k}$. These $z$ embeddings for the entire $2N$ batch are then subjected to a contrastive loss similar to above. This enables us to maximize the mutual information between the underlying video data and the joint distribution of the 2D and 3D embeddings to eventually learn highly generalizable feature representations. It further encourages the interaction between the two streams to improve representation learning while being jointly trained end-to-end.

\paragraph{Joint Contrastive Loss} The embeddings, $h^{ap}_{2k}$ and $h^{act}_{2k}$, obtained from the 2D and 3D encoder streams respectively help us to separately encode the visual information of the video independently and also jointly with the temporal information of the video. However, in order to learn highly generalizable feature representations that can adapt to novel classes in very few samples, it is important to also maximize the mutual information between the underlying video data and the joint distribution of the 2D and 3D embeddings. We therefore introduce a third non-linear MLP projection head that takes the concatenation of $h^{ap}_{2k}$ and $h^{act}_{2k}$ as input to output $z^{joint}_{2k}$. The $z^{joint}$ embeddings for the entire $2N$ batch are subjected to a contrastive loss, $\mathcal{L}^{joint}_{NCE}$, similar to above. This joint contrastive loss encourages the interaction and information pooling of complimentary features between the two streams to improve representation learning of our end-to-end jointly trained model.

\paragraph{Symmetric KL Divergence} To further enforce coherence between the 2D and 3D modalities and minimize redundancy between the information encoded in the corresponding embeddings for each modality, we further minimize the symmetric KL divergence, $D_{SKL}$, between the 2D and 3D encoding distributions~\cite{federici2019learning, wei2020co2}. Since $D_{SKL}$ requires the embeddings as probability distributions, we consider the softmax probabilities coming out of the 2D- and 3D-stream specific MLP projection heads as the probability distributions of the 2D and 3D embeddings respectively. The softmax probabilities can be interpreted as the probability of a query $z_i$ to correctly match its positive twin $z_j$ from the rest of $2N-1$ samples in the batch. This formulation has an added benefit over explicitly reparameterizing the $z$ or $h$ embedding as it does not enforce a prior on the distribution such as the Gaussian prior.

Based on the above, the final loss, $\mathcal{L}^{MM}_{NCE}$, used to train \methodname~ end-to-end in a self-supervised manner over the unlabeled video data is given as,
\begin{equation}
    \mathcal{L}^{MM}_{NCE}  = \mathcal{L}^{ap}_{NCE} + \mathcal{L}^{act}_{NCE} + \mathcal{L}^{joint}_{NCE} + D_{SKL}(P^{ap} || P^{act})
\end{equation}



%In our MM-NCE loss to maximize mutual information between the embeddings and the video data, we generate multiple diverse views/augmentations that are tailored to capture different aspects of the video data. For the 2D-appearance stream, since there is more focus on the spatial visual information independent of the temporal information of the video, the views are individual video frames that are randomly sampled from the entire span of the video. Moreover, we consider a higher resolution~$(224 \times 224)$ for these views to increase the visual information encoded by the latent representations of the 2D-stream. To spatially augment the frames, we follow the augmentation protocol from SimCLR.


%\subsection{Augmentation}
%In our MM-NCE loss to maximize mutual information between the embeddings and the video data, we generate multiple diverse views/augmentations that are tailored to capture different aspects of the video data. For the 2D-appearance stream, since there is more focus on the spatial visual information independent of the temporal information of the video, the views are individual video frames that are randomly sampled from the entire span of the video. Moreover, we consider a higher resolution~$(224 \times 224)$ for these views to increase the visual information encoded by the latent representations of the 2D-stream. To spatially augment the frames, we follow the augmentation protocol from SimCLR.

%On the other hand, for the 3D-action stream, the emphasis is to encode spatio-temporal action information of the video, \ie, visual information in conjunction with the temporal information. Therefore, the views are considered as an aggregation of one or more video frames. The frames forming these video segments are temporally ordered and can be sampled as per different protocols such as random, temporally segmented [] or uniformly sampled with one or more stride. To strike a better balance between the encoded spatial and temporal information, we consider a lower image resolution~$(112 \times 112)$ for each sampled frame. We follow the temporally consistent spatial augmentation protocol from CVRL to further augment these sampled video segments before feeding them to the 3D-encoder stream.

% \begin{algorithm}[t]
% \label{algo:offline}
% \caption{\methodname: Self-supervised Training}
% \end{algorithm}
\subsection{Few shot Meta-Testing}
As illustrated in Fig~\ref{fig:sesumi_model} (b) we follow the transfer learning approach by way of finetuning our representations with a linear classifier. The support and query videos undergo the action sampling (4x4) and  appearance sampling (8x1) similar to training. After resizing the inputs they are CenterCropped. The projection heads are discarded during testing and the L-2 normalized embeddings from the appearance and action streams are concatenated and fed as inputs to a linear N-way classifier trained with cross-entropy loss.

% \subsection{Few shot Meta-Testing}As illustrated Fig~\ref{fig:sesumi_model} (b) we follow the transfer learning approach by way of finetuning our representations with a linear classifier  The  action sampling (4x4) and  appearance sampling (8x1) for the support and query videos, input frame resolutions are consistent with training however the augmentations are  composed of  Resizing and CenterCroping. The projection heads are discarded during testing and the L-2 normalized embeddings from the appearance and action streams are concatenated and fed as inputs to a linear N-way classifier trained with cross-entropy loss.
 
% We build our self-supervised framework of contrastive
% video representation learning (CVRL) upon SimCLR \cite{chen2020simple} in
% view of its simplicity and compelling performance on learning image representations.

% The core of this framework is an InfoNCE contrastive
% loss [36] applied on features extracted from augmented
% videos. Suppose we sample N videos per mini-batch and
% augment them, resulting in 2N videos (the augmentation
% module is described in Section 3.3). Denote by zi z
% 0
% i
% the
% encoded representations of the two augmented versions of
% the i-th input video


% \begin{figure}[t]
% \begin{center}
% \fbox{\rule{0pt}{2in} \rule{0.9\linewidth}{0pt}}
%   %\includegraphics[width=0.8\linewidth]{egfigure.eps}
% \end{center}
%   \caption{Example of caption.  It is set in Roman so that mathematics
%   (always set in Roman: $B \sin A = A \sin B$) may be included without an
%   ugly clash.}
% \label{fig:long}
% \label{fig:onecol}
% \end{figure}




==> sections/related_work_bkp.tex <==
\section{Related Work}
In a standard few-shot learning protocol, there is a set of \textit{base} classes with relatively large number of labeled samples and a set of \textit{novel} classes with samples that are unseen to the model. The \textit{base} class data is used to train the model in a \textit{meta-training} phase to learn to classify using as few reference samples as possible. The model is then evaluated in a \textit{meta-testing} phase where it classifies samples~(query) from a subset of the novel classes based on few (typically one or five) labeled examples~(support). 
 
\textbf{Few-Shot Learning} 
 Metric learning approaches ~\cite{snell2017prototypical, vinyals2016matching, sung2018learning} aim to minimizes the distance between support and query embeddings or parametrize the similarity between them. Meta-learning~\cite{finn2017model, ravi2016optimization} develop rapidly learnable models in a  `learn-to-learn' paradigm for efficient adaptation on novel classes. Limits on base-class data size have inspired some approaches to use data augmentation or data hallucination \cite{wang2018low,hariharan2017low}. Recent work on non-episodic few-shot learning \cite{wang2019simpleshot,chen2019closer, xian2020generalized} show that  state-of-the-art performance can be obtained by training larger models and dataset. Attention mechanisms \cite{gidaris2018dynamic}, especially cross-attention have shown to be quite effective \cite{hou2019cross, doersch2020crosstransformers},  which we also utilize in \methodname~as part of A3M. 
 
 \textbf{Unsupervised Few-Shot Learning}
 Leveraging unlabeled data in addition to base-class data using auxiliary self-supervision has shown to boost few-shot performance~\cite{gidaris2019boosting, ren2018meta, doersch2020crosstransformers}. Recently unsupervised meta-learning approaches for few-shot image classification~\cite{khodadadeh2019unsupervised,  medina2020self, hsu2018unsupervised} have shown competitive performance without using base class labels.
 %Similar to these works, we acquire task-specific few-shot priors by generating episodes from unlabelled data, however to solve a more challenging problem in videos. 
 
 
\textbf{Action Recognition}
For action recognition, there are both 2D models that operate on a per-frame basis with temporal feature aggregation~\cite{girdhar2017actionvlad, feichtenhofer2019slowfast} and 3D models~\cite{hara2017learning,tran2015learning} that capture spatio-temporal features. The major issue with 2D models is a lack of long-term temporal reasoning, and with 3D models, there is often overfitting due to the large number of  trainable parameters.
To alleviate the problem of capturing  long-term dependencies, self-attention mechanisms~\cite{wang2018non} and temporal relation modules \cite{zhou2018temporal} have shown success.  To improve parameter efficiency, recent methods have looked at factorizing 3D convolutions~\cite{tran2018closer}, replacement of costly 3D operations with 2D replacements~\cite{xie2018rethinking} or just using 2D CNN in a slow-fast setting~\cite{feichtenhofer2019slowfast}. Two-stream methods~\cite{wang2016temporal,carreira2017quo}  exploit optical flow along with RGB sequences to  acquire complementary information. 

\textbf{Unsupervised Video Representation Learning}
Solving pretext tasks in images \cite{doersch2015unsupervised,zhang2016colorful,gidaris2018unsupervised, noroozi2016unsupervised} has inspired methods to learn from videos in an unsupervised manner~\cite{jing2018self, kim2019self}. Pretext tasks in video can include time or video dynamics as supervisory signal like sorting frames, clip order frame prediction, frame sampling, speediness, \etc~\cite{misra2016shuffle, lee2017unsupervised, xu2019self, wang2020self, benaim2020speednet, lotter2016deep, han2020memory, piergiovanni2020evolving}. Recently, methods employing contrastive learning~(InfoNCE)~\cite{oord2018representation} have been the most effective in harnessing large-scale unlabeled data~\cite{he2020momentum, chen2020simple, qian2020spatiotemporal, tao2020self,  Han20CoCLR} and perform comparably to supervised methods on vision tasks. Although these methods have show low-shot learning capabilites, it is primarily limited to being able to finetune on in-distribution training classes with a tiny fraction of full-labeled dataset. Without any dedicated few-shot meta-learning mechanism during training, the existing unsupervised methods still require a full-size labeled dataset to optimally transfer to a downstream task with out-of-distribution novel classes.

% Recently, contrastive learning techniques provide a more effective way to learn video semantics without pre-defined tasks or puzzle solving \cite{qian2020spatiotemporal, tao2020self,  Han20CoCLR}. 

\begin{figure*}[t]
\begin{center}
%\fbox{\rule{0pt}{2in} \rule{0.9\linewidth}{0pt}}
   \includegraphics[width=\textwidth]{sections/figures/model_diagram_meta_uvfs_full_2.pdf}
\end{center}
   \caption{\methodname: Model Overview. (a) \textbf{Two-stream Training}: using a large unlabeled video dataset subjected to our sampling and augmentation scheme (see Section~\ref{sec:sampling}).  (b) \textbf{Episode Generation} hard episodes are mined from the unsupervised features.  (c) \textbf{A3M} module learns to align appearance over action features through meta-adaption on hard episodes.  (d) \textbf{Meta-testing} A3M as a few-shot classifier finetunes on novel class support to classify query videos.}
\label{fig:sesumi_model}
\vspace{-1em}
\end{figure*}

\textbf{Few Shot Video Action Recognition}
 ProtoGAN \cite{kumar2019protogan} synthesizes additional examples for novel class support with a conditional generative adversarial network. 
 CMN \cite{zhu2018compound} has  a multi-saliency algorithm to store video features in a compound memory network to classify by matching queries. TARN and ARN \cite{bishay2019tarn, zhang2020few} capture spatio-temporal dependencies using attention mechanisms. In OTAM \cite{Cao_2020_CVPR} a deep distance metric generates a matching score for query-support pairs that maintain the frame order.   R-3DFSV \cite{xian2020generalized} train large pretrained 3D CNN backbone  and augment novel class support with weak labels. RVN \cite{cao2020few} models the 
 query support feature alignment via LSTMs to optimize similarity scores. AMeFu-Net \cite{fu2020depth} fuses depth with RGB as an additional modality to align appearance and motion information.  In constrast to all of these previous methods utilizing labeled supervision during `meta-training', our proposed method, \methodname, is completely unsupervised. 


==> sections/training_classes.tex <==
\subsection{Class Removal for Kinetics700}

% abseiling,
% acting in play,
% adjusting glasses,
% air drumming,
% alligator wrestling,
% answering questions,
% applauding,
% applying cream,
% archaeological excavation,
% archery,
% arguing,
% arm wrestling,
% arranging flowers,
% arresting,
% assembling bicycle,
% assembling computer,
% attending conference,
% auctioning,
% baby waking up,
% backflip (human),
% bandaging,
% barbequing,
% bartending,
% base jumping,
% bathing dog,
% battle rope training,
% beatboxing,
% bee keeping,
% being excited,
% being in zero gravity,
% belly dancing,
% bench pressing,
% bending back,
% bending metal,
% biking through snow,
% blending fruit,
% blowdrying hair,
% blowing bubble gum,
% blowing glass,
% blowing leaves,
% blowing nose,
% blowing out candles,
% bobsledding,
% bodysurfing,
% bookbinding,
% bottling,
% bouncing ball (not juggling),
% bouncing on bouncy castle,
% bouncing on trampoline,
% bowling,
% braiding hair,
% breading or breadcrumbing,
% breakdancing,
% breaking boards,
% breaking glass,
% breathing fire,
% brush painting,
% brushing floor,
% brushing hair,
% brushing teeth,
% building cabinet,
% building lego,
% building sandcastle,
% building shed,
% bulldozing,
% bungee jumping,
% burping,
% calculating,
% calligraphy,
% canoeing or kayaking,
% capoeira,
% capsizing,
% card stacking,
% card throwing,
% carrying baby,
% carrying weight,
% cartwheeling,
% carving ice,
% carving marble,
% carving pumpkin,
% carving wood with a knife,
% casting fishing line,
% catching fish,
% catching or throwing baseball,
% catching or throwing frisbee,
% catching or throwing softball,
% celebrating,
% changing gear in car,
% changing oil,
% changing wheel (not on bike),
% chasing,
% checking tires,
% checking watch,
% cheerleading,
% chewing gum,
% chiseling stone,
% chiseling wood,
% chopping meat,
% chopping wood,
% clam digging,
% clapping,
% clay pottery making,
% cleaning gutters,
% cleaning pool,
% cleaning shoes,
% cleaning toilet,
% cleaning windows,
% climbing a rope,
% climbing ladder,
% climbing tree,
% closing door,
% coloring in,
% combing hair,
% contact juggling,
% contorting,
% cooking chicken,
% cooking egg,
% cooking on campfire,
% cooking sausages (not on barbeque),
% cooking scallops,
% cosplaying,
% coughing,
% counting money,
% country line dancing,
% cracking back,
% cracking knuckles,
% cracking neck,
% crawling baby,
% crocheting,
% crossing eyes,
% crying,
% cumbia,
% curling (sport),
% curling eyelashes,
% curling hair,
% cutting apple,
% cutting cake,
% cutting nails,
% cutting orange,
% cutting pineapple,
% dancing gangnam style,
% deadlifting,
% dealing cards,
% decorating the christmas tree,
% decoupage,
% delivering mail,
% digging,
% dining,
% directing traffic,
% disc golfing,
% docking boat,
% dodgeball,
% doing aerobics,
% doing jigsaw puzzle,
% doing laundry,
% doing nails,
% doing sudoku,
% drawing,
% dribbling basketball,
% drinking shots,
% driving car,
% driving tractor,
% drooling,
% drop kicking,
% drumming fingers,
% dumpster diving,
% dyeing eyebrows,
% dyeing hair,
% eating burger,
% eating cake,
% eating carrots,
% eating chips,
% eating doughnuts,
% eating hotdog,
% eating ice cream,
% eating nachos,
% eating spaghetti,
% eating watermelon,
% egg hunting,
% embroidering,
% entering church,
% exercising arm,
% exercising with an exercise ball,
% extinguishing fire,
% faceplanting,
% falling off bike,
% falling off chair,
% feeding birds,
% feeding goats,
% fencing (sport),
% fidgeting,
% filling cake,
% finger snapping,
% fixing bicycle,
% fixing hair,
% flint knapping,
% flipping bottle,
% flipping pancake,
% fly tying,
% folding clothes,
% folding napkins,
% front raises,
% frying vegetables,
% gargling,
% geocaching,
% getting a haircut,
% getting a piercing,
% getting a tattoo,
% giving or receiving award,
% gold panning,
% golf chipping,
% golf driving,
% golf putting,
% gospel singing in church,
% grinding meat,
% grooming cat,
% grooming dog,
% grooming horse,
% hand washing clothes,
% head stand,
% headbanging,
% headbutting,
% helmet diving,
% herding cattle,
% high fiving,
% historical reenactment,
% hitting baseball,
% hockey stop,
% holding snake,
% home roasting coffee,
% hopscotch,
% hoverboarding,
% huddling,
% hugging (not baby),
% hugging baby,
% hurdling,
% ice climbing,
% ice fishing,
% ice swimming,
% inflating balloons,
% installing carpet,
% ironing,
% ironing hair,
% jaywalking,
% jetskiing,
% jogging,
% juggling balls,
% juggling fire,
% juggling soccer ball,
% jumping bicycle,
% jumping into pool,
% jumping jacks,
% jumping sofa,
% jumpstyle dancing,
% karaoke,
% kicking field goal,
% kicking soccer ball,
% kissing,
% kitesurfing,
% knitting,
% krumping,
% land sailing,
% laughing,
% lawn mower racing,
% laying bricks,
% laying concrete,
% laying decking,
% laying stone,
% laying tiles,
% leatherworking,
% letting go of balloon,
% licking,
% lifting hat,
% lighting candle,
% lighting fire,
% listening with headphones,
% lock picking,
% long jump,
% longboarding,
% looking at phone,
% looking in mirror,
% luge,
% lunge,
% making a cake,
% making a sandwich,
% making balloon shapes,
% making bubbles,
% making cheese,
% making horseshoes,
% making jewelry,
% making latte art,
% making paper aeroplanes,
% making pizza,
% making slime,
% making snowman,
% making sushi,
% making tea,
% making the bed,
% marching,
% marriage proposal,
% massaging back,
% massaging feet,
% massaging legs,
% massaging neck,
% "massaging persons head",
% metal detecting,
% milking cow,
% milking goat,
% mixing colours,
% moon walking,
% mopping floor,
% mosh pit dancing,
% motorcycling,
% mountain climber (exercise),
% moving baby,
% moving child,
% moving furniture,
% mowing lawn,
% mushroom foraging,
% needle felting,
% news anchoring,
% packing,
% parasailing,
% parkour,
% passing American football (in game),
% passing American football (not in game),
% passing soccer ball,
% peeling apples,
% peeling banana,
% peeling potatoes,
% person collecting garbage,
% petting animal (not cat),
% petting cat,
% petting horse,
% photobombing,
% photocopying,
% picking apples,
% picking blueberries,
% pillow fight,
% pinching,
% pirouetting,
% planing wood,
% planting trees,
% plastering,
% playing accordion,
% playing american football,
% playing badminton,
% playing bagpipes,
% playing basketball,
% playing beer pong,
% playing billiards,
% playing blackjack,
% playing cards,
% playing cello,
% playing checkers,
% playing chess,
% playing clarinet,
% playing controller,
% playing cymbals,
% playing darts,
% playing didgeridoo,
% playing dominoes,
% playing field hockey,
% playing flute,
% playing gong,
% playing hand clapping games,
% playing harmonica,
% playing harp,
% playing ice hockey,
% playing keyboard,
% playing kickball,
% playing laser tag,
% playing lute,
% playing mahjong,
% playing maracas,
% playing marbles,
% playing netball,
% playing nose flute,
% playing oboe,
% playing ocarina,
% playing organ,
% playing paintball,
% playing pan pipes,
% playing piano,
% playing piccolo,
% playing pinball,
% playing ping pong,
% playing poker,
% playing polo,
% playing recorder,
% playing road hockey,
% playing rounders,
% playing rubiks cube,
% playing saxophone,
% playing scrabble,
% playing shuffleboard,
% playing slot machine,
% playing squash or racquetball,
% playing ukulele,
% playing violin,
% playing with trains,
% playing xylophone,
% poaching eggs,
% pole vault,
% polishing furniture,
% polishing metal,
% popping balloons,
% preparing salad,
% presenting weather forecast,
% pretending to be a statue,
% pull ups,
% pulling espresso shot,
% pulling rope (game),
% pumping fist,
% pumping gas,
% punching person (boxing),
% pushing cart,
% pushing wheelbarrow,
% pushing wheelchair,
% putting in contact lenses,
% putting on eyeliner,
% putting on foundation,
% putting on mascara,
% putting on sari,
% putting on shoes,
% raising eyebrows,
% reading book,
% reading newspaper,
% recording music,
% repairing puncture,
% riding a bike,
% riding camel,
% riding mechanical bull,
% riding mule,
% riding scooter,
% riding snow blower,
% riding unicycle,
% ripping paper,
% roasting marshmallows,
% roasting pig,
% robot dancing,
% rock scissors paper,
% roller skating,
% rolling eyes,
% rolling pastry,
% rope pushdown,
% running on treadmill,
% sailing,
% saluting,
% sanding floor,
% sanding wood,
% sausage making,
% sawing wood,
% scrambling eggs,
% scrapbooking,
% scrubbing face,
% seasoning food,
% separating eggs,
% setting table,
% sewing,
% shaking hands,
% shaking head,
% shaping bread dough,
% sharpening knives,
% sharpening pencil,
% shaving head,
% shaving legs,
% shining flashlight,
% shining shoes,
% shoot dance,
% shooting basketball,
% shooting goal (soccer),
% shooting off fireworks,
% shopping,
% shouting,
% shoveling snow,
% shredding paper,
% shucking oysters,
% shuffling cards,
% shuffling feet,
% sieving,
% sign language interpreting,
% silent disco,
% singing,
% sipping cup,
% situp,
% skipping stone,
% slacklining,
% slapping,
% sled dog racing,
% sleeping,
% slicing onion,
% smashing,
% smelling feet,
% smoking,
% smoking hookah,
% smoking pipe,
% snatch weight lifting,
% sneezing,
% snorkeling,
% snowboarding,
% snowkiting,
% snowmobiling,
% somersaulting,
% spelunking,
% spinning plates,
% spinning poi,
% splashing water,
% spray painting,
% spraying,
% square dancing,
% squat,
% stacking cups,
% stacking dice,
% staring,
% steer roping,
% steering car,
% sticking tongue out,
% stomping grapes,
% stretching leg,
% sucking lolly,
% surfing crowd,
% surveying,
% sweeping floor,
% swimming backstroke,
% swimming breast stroke,
% swimming butterfly stroke,
% swimming front crawl,
% swimming with dolphins,
% swimming with sharks,
% swing dancing,
% swinging baseball bat,
% swinging on something,
% sword fighting,
% sword swallowing,
% tackling,
% tagging graffiti,
% tai chi,
% taking photo,
% talking on cell phone,
% tango dancing,
% tapping guitar,
% tapping pen,
% tasting beer,
% tasting food,
% tasting wine,
% testifying,
% texting,
% threading needle,
% throwing ball (not baseball or American football),
% throwing discus,
% throwing knife,
% throwing snowballs,
% throwing tantrum,
% throwing water balloon,
% tickling,
% tie dying,
% tightrope walking,
% tiptoeing,
% tobogganing,
% tossing coin,
% tossing salad,
% training dog,
% trapezing,
% treating wood,
% trimming shrubs,
% trimming trees,
% triple jump,
% twiddling fingers,
% tying bow tie,
% tying knot (not on a tie),
% tying necktie,
% tying shoe laces,
% uncorking champagne,
% unloading truck,
% using a microscope,
% using a power drill,
% using a sledge hammer,
% using a wrench,
% using atm,
% using bagging machine,
% using circular saw,
% using inhaler,
% using megaphone,
% using puppets,
% using remote controller (not gaming),
% using segway,
% vacuuming car,
% vacuuming floor,
% visiting the zoo,
% wading through mud,
% wading through water,
% waiting in line,
% waking up,
% walking on stilts,
% walking the dog,
% walking through snow,
% walking with crutches,
% washing dishes,
% washing feet,
% washing hair,
% washing hands,
% watching tv,
% water skiing,
% water sliding,
% watering plants,
% waving hand,
% waxing armpits,
% waxing back,
% waxing chest,
% waxing eyebrows,
% waxing legs,
% weaving basket,
% weaving fabric,
% welding,
% whistling,
% windsurfing,
% winking,
% wood burning (art),
% wrapping present,
% wrestling,
% writing,
% yarn spinning,
% yawning,
% yoga,
% zumba.

% \subsection{Kinetics100}
% air drumming,
% arm wrestling,
% beatboxing,
% biking through snow,
% blowing glass,
% bowling,
% breakdancing,
% bungee jumping,
% catching or throwing baseball,
% cheerleading,
% cleaning floor,
% contact juggling,
% cooking chicken,
% country line dancing,
% curling hair,
% deadlifting,
% doing nails,
% dribbling basketball,
% driving tractor,
% drop kicking,
% dying hair,
% eating burger,
% feeding birds,
% giving or receiving award,
% hopscotch,
% jetskiing,
% jumping into pool,
% laughing,
% making snowman,
% massaging back,
% mowing lawn,
% opening bottle,
% playing accordion,
% playing badminton,
% playing basketball,
% playing didgeridoo,
% playing ice hockey,
% playing keyboard,
% playing ukulele,
% playing xylophone,
% presenting weather forecast,
% punching bag,
% pushing cart,
% reading book,
% riding unicycle,
% shaking head,
% sharpening pencil,
% shaving head,
% shot put,
% shuffling cards,
% slacklining,
% sled dog racing,
% snowboarding,
% somersaulting,
% squat,
% surfing crowd,
% trapezing,
% using computer,
% washing dishes,
% washing hands,
% water skiing,
% waxing legs,
% weaving basket,

We remove the following 58 classes from Kinetics700 dataset:\\
blasting sand,
 busking,
 clean and jerk,
 cutting watermelon,
 dancing ballet,
 dancing charleston,
 dancing macarena,
 diving cliff,
 fencing (sport),
 filling eyebrows,
 folding paper,
 gymnastics tumbling,
 high jump,
 high kick,
 hula hooping,
 hurling (sport),
 ice skating,
 kicking field goal,
 kicking soccer ball,
 paragliding,
 playing drums,
 playing kickball,
 playing monopoly,
 playing tennis,
 playing trumpet,
 playing volleyball,
 pouring beer,
 pouring milk,
 pouring wine,
 punching bag,
 punching person (boxing),
 push up,
 pushing car,
 riding elephant,
 riding or walking with horse,
 rock climbing,
 running on treadmill,
 salsa dancing,
 shearing sheep,
 side kick,
 ski ballet,
 ski jumping,
 skiing crosscountry,
 skiing mono,
 skiing slalom,
 skipping rope,
 skydiving,
 smoking,
 smoking hookah,
 smoking pipe,
 springboard diving,
 standing on hands,
 stretching arm,
 surfing water,
 talking on cell phone,
 tap dancing,
 throwing axe,
 unboxing.

\subsection{Class Removal for UCF101}
We remove 4 base classes from UCF101 split: \\
Drumming, PushUps, Fencing, WallPushups. 
% ApplyEyeMakeUp, Archery,
% BabyCrawling, BalanceBeam, BandMarching, BaseballPitch, Basketball, BasketballDunk, BenchPress, Biking,
% Billiards, BlowDryHair, BodyWeightSquats, Bowling,
% BoxingPunchingBag, BoxingSpeedBag, BreastStroke,
% BrushingTeeth, CricketBowling,  ,
% FieldHockeyPenalty, FrisbeeCatch, FrontCrawl, Haircut,
% Hammering, HeadMassage, HulaHoop, JavelinThrow, JugglingBalls, JumpingJack, Kayaking, Knitting, LongJump,
% Lunges, MilitaryParade, Mixing, MoppingFloow,
% Nunchucks, ParallelBars, PizzaTossing, PlayingCello,
% PlayingDhol, PlayingFlute, PlayingPiano, PlayingSitar, PlayingTabla, PlayingViolin, PoleVault, Pullups,
%  Rafting, RopeClimbing, Rowing, ShavingBeard,
% Skijet, SoccerJuggling, SoccerPenalty, SumoWrestling,
% Swing, TableTennisShot, Taichi, ThrowDiscus, TrampolineJumpling, Typing, UnevenBars, WalkingWithDog,
%  WritingOnBoard, YoYo

% remove from kinetics
% Drumming,
% remove from hmdb51
% PushUps, Fencing
% WallPushups ?

\subsection{Class Removal for HMDB51}
We remove 4 base classes from HMDB51 split: \\
punch, handstand, push, throw


\subsection{Class Removal for Kinetics100}
We remove 1 base classes from Kinetics100 split: \\
blowing candles
% brush hairs, catch, chew, clap,
% climb, climb stairs,   draw sword, dribble, drink, fall
% floor, flic flac,  hug, jump, kiss, pullup, punch,
% push, ride bike, ride horse, shake hands, shoot bow, situp,
% stand, sword, sword exercies, throw, turn, walk, wave.


% ucf101
% punch-

% --> doubtfull
% handstand- > HandstandWalking 

% k100
% push -> pushing car
% throw -> throwing axes


==> tables/Dataset.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage{graphicx}
% \begin{table}[t]
% \begin{center}
% \resizebox{\textwidth}{!}{%
% \begin{tabular}{|l|c|c|c|c|c|c|}
% \hline
% \multirow{2}{*}{Methods} & \multicolumn{2}{c|}{UCF101} & \multicolumn{2}{c|}{HMDB51} & \multicolumn{2}{c|}{Kinetics100} \\ \cline{2-7} 
%  & 1-shot & 5-shot & 1-shot & 5-shot & 1-shot & 5-shot \\ \hline
% Base Class Data & - & - & - & - &  &  \\ \hline
% k700 & - & - & - & - &  &  \\ \hline
% 1\% Supervision &  &  &  &  &  & \\ \hline
% \end{tabular}%
% }
% \caption{Performance with data ablations}
% \label{tab:data}
% \end{table}

% \begin{table}[]
% \begin{tabular}{lllllll}
% \hline
% \textbf{} & \multicolumn{2}{c}{\textbf{UCF101}} & \multicolumn{2}{c}{\textbf{HMDB51}} & \multicolumn{2}{c}{\textbf{Kinetics100}} \\ \hline
%  & \multicolumn{1}{c}{\textbf{1 Shot}} & \multicolumn{1}{c}{\textbf{5 Shot}} & \multicolumn{1}{c}{\textbf{1 Shot}} & \multicolumn{1}{c}{\textbf{5 Shot}} & \multicolumn{1}{c}{\textbf{1 Shot}} & \multicolumn{1}{c}{\textbf{5 Shot}} \\ \hline
% Base Class only & {\color[HTML]{FE0000} \textbf{0.07}} & {\color[HTML]{FE0000} \textbf{0.15}} & {\color[HTML]{00009B} \textbf{0.18}} & {\color[HTML]{00009B} \textbf{0.22}} & {\color[HTML]{FE0000} \textbf{0.16}} & {\color[HTML]{FE0000} \textbf{0.19}} \\
% +Kinetics700 & 0.17 & 0.27 & 0.43 & 0.41 & 0.38 & 0.38 \\
% + 1\% base labels  & 0.12 & 0.42 & 0.21 & 0.37 & 0.36 & 0.47 \\ \hline
% \textbf{Ours} & {\color[HTML]{00009B} \textbf{0.11}} & {\color[HTML]{00009B} \textbf{0.24}} & {\color[HTML]{FE0000} \textbf{0.08}} & {\color[HTML]{FE0000} \textbf{0.17}} & {\color[HTML]{00009B} \textbf{0.21}} & {\color[HTML]{00009B} \textbf{0.28}} \\ \hline
% \end{tabular}
% \caption{  }
% \label{tab:leaderboard}
% \end{table}

% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[h]
\begin{tabular}{|l|l|l|l|l|l|l|}
\hline
\multicolumn{1}{|c|}{\multirow{2}{*}{Baselines}} & \multicolumn{2}{c|}{UCF101} & \multicolumn{2}{c|}{HMDB51} & \multicolumn{2}{c|}{Kinetics100} \\ \cline{2-7} 
\multicolumn{1}{|c|}{} & \multicolumn{1}{c|}{1 Shot} & \multicolumn{1}{c|}{5 Shot} & \multicolumn{1}{c|}{1 Shot} & \multicolumn{1}{c|}{5 Shot} & \multicolumn{1}{c|}{1 Shot} & \multicolumn{1}{c|}{5 Shot} \\ \hline
Base Class only &  &  &  &  &  &  \\ \hline
+Kinetics700 &  &  &  &  &  &  \\ \hline
% + 1\% base labels &  &  &  &  &  &  \\ \hline
\end{tabular}
\caption{Comparison of VideoCLR across dataset splits.}
\label{tab:databaselines}
\end{table*}

==> tables/FSVAR.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
\begin{table*}[t]
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{|l|c|c|c|c|c|c|c|c|}
\hline
\multirow{2}{*}{Methods} & \multicolumn{2}{c|}{Supervision} & \multicolumn{2}{c|}{UCF101} & \multicolumn{2}{c|}{HMDB51} & \multicolumn{2}{c|}{Kinetics100} \\ \cline{2-9} 
 & \multicolumn{1}{l|}{Sup. Pretraining} & \multicolumn{1}{l|}{Base Sup.} & 1-shot & 5-shot & 1-shot & 5-shot & 1-shot & 5-shot \\ \hline
Matching Net \cite{zhu2018compound} & Imagenet-2D & Yes & - & - & - & - & 53.3 & 74.6 \\ 
MAML \cite{zhu2018compound} & Imagenet-2D & Yes & - & - & - & - & 54.2 & 75.3 \\ 
CMN \cite{zhu2018compound} & Imagenet-2D & Yes & - & - & - & - & 60.5 & 78.9 \\ 
TARN \cite{bishay2019tarn} & Sports-1M & Yes & - & - & - & - & 66.6 & 80.7 \\ 
OTAM \cite{Cao_2020_CVPR} & Imagenet-2D & Yes & - & - & - & - & 73.0 & 85.8 \\
R-3DFSV  \cite{xian2020generalized} & Sports-1M & Yes & - & - & - & - & 95.3 & 97.8 \\ 
ProtoGAN \cite{kumar2019protogan} & Sports-1M  & Yes  & 57.8 ± 3.0 & 80.2 ± 1.3 & 34.7 ± 9.20 & 54.0 ± 3.90 & - & - \\ 
AmeFu-Net \cite{fu2020depth} & Imagenet-2D & Yes & 85.1 & 95.5 & 60.2 & 75.  & 74.1  & 86.8 \\ 
RVN \cite{cao2020few} & Kinetics-400 & Yes  & 88.71 ± 0.19 & 96.78 ± 0.08 & 63.43 ± 0.28 & 79.69 ± 0.20 & - & - \\ \hline
ARN  \cite{zhang2020few}  & No & Yes & 66.32 ± 0.99 & 83.12 ± 0.70 & 45.15 ± 0.96 & 60.56 ± 0.86 & 63.7 & 82.4 \\ 

% \methodname~(Ours) (3D stream only)  & No & No & 63.0 ±  &  87.8 ± 0.15  & 44.21 ± & 60.35 ±  0.23  & 53.26±0.24 & 71.39±0.22\\ 
\methodname~(Ours)  & No & No & \textbf{73.41 ± 0.24}  & \textbf{91.29 ± 0.14} & \textbf{47.21 ± 0.23}  &  \textbf{65.28 ± 0.28} & \textbf{61.61 ± 0.46} & \textbf{79.20 ± 0.39} \\ 

\methodname~(ProtoNet~\cite{snell2017prototypical})  & No & No & 42.47 ± 0.42  &  & 36.01 ± 0.40 &   & 31.20 ± 0.39 & \\ 
\methodname~(Baseline++~\cite{chen2018closer}) & No & No & 70.42 ± 0.45 &  & 42.98 ± 0.47 &  & 56.10 ± 0.47 &  \\ 
\hline


\end{tabular}%
}
\caption{Few-shot video classification results. We report 5-way video classification accuracy on meta-testing set. Our approach surpasses previous supervised state-of-the-arts by a large margin.}
\label{tab:fsvar}

\end{table*}

% \begin{figure*}
% \begin{center}
% \fbox{\rule{0pt}{2in} \rule{.9\linewidth}{0pt}}
% \end{center}
%   \caption{Example of a short caption, which should be centered.}
% \label{fig:short}
% \end{figure*}


% \begin{table}
% \begin{center}
% \begin{tabular}{|l|c|}
% \hline
% Method & Frobnability \\
% \hline\hline
% Theirs & Frumpy \\
% Yours & Frobbly \\
% Ours & Makes one's heart Frob\\
% \hline
% \end{tabular}
% \end{center}
% \caption{Results.   Ours is better.}
% \end{table}


==> tables/FSVAR_SS+ablations.tex <==
\begin{table*}[t]
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{|l|c|c|c|c|c|c|c|c|}
\hline
\multirow{2}{*}{Methods} & \multicolumn{2}{c|}{Supervision} & \multicolumn{2}{c|}{UCF101} & \multicolumn{2}{c|}{HMDB51} & \multicolumn{2}{c|}{Kinetics100} \\ \cline{2-9} 
 & \multicolumn{1}{l|}{Sup. Pretraining} & \multicolumn{1}{l|}{Base Sup.} & 1-shot & 5-shot & 1-shot & 5-shot & 1-shot & 5-shot \\ \hline
Matching Net \cite{zhu2018compound} & Imagenet-2D & Yes & - & - & - & - & 53.3 & 74.6 \\ 
MAML \cite{zhu2018compound} & Imagenet-2D & Yes & - & - & - & - & 54.2 & 75.3 \\ 
CMN \cite{zhu2018compound} & Imagenet-2D & Yes & - & - & - & - & 60.5 & 78.9 \\ 
TARN \cite{bishay2019tarn} & Sports-1M & Yes & - & - & - & - & 66.6 & 80.7 \\ 
OTAM \cite{Cao_2020_CVPR} & Imagenet-2D & Yes & - & - & - & - & 73.0 & 85.8 \\
R-3DFSV  \cite{xian2020generalized} & Sports-1M & Yes & - & - & - & - & 95.3 & 97.8 \\ 
ProtoGAN \cite{kumar2019protogan} & Sports-1M  & Yes  & 57.8 ± 3.0 & 80.2 ± 1.3 & 34.7 ± 9.20 & 54.0 ± 3.90 & - & - \\ 
AmeFu-Net \cite{fu2020depth} & Imagenet-2D & Yes & 85.1 & 95.5 & 60.2 & 75.  & 74.1  & 86.8 \\ 
RVN \cite{cao2020few} & Kinetics-400 & Yes  & 88.71 ± 0.19 & 96.78 ± 0.08 & 63.43 ± 0.28 & 79.69 ± 0.20 & - & - \\ \hline
ARN  \cite{zhang2020few}  & No & Yes & 66.32 ± 0.99 & 83.12 ± 0.70 & 45.15 ± 0.96 & 60.56 ± 0.86 & 63.7 & 82.4 \\ \hline

3DRotNet \cite{jing2018self} & No & No & 38.43+0.23	& 33.61+0.15 & 27.35+ 0.2 & 26.84+0.13 & 27.53+ 0.2 &	25.54+0.13 \\ 
VCOP \cite{xu2019self}  & No & No & 32.91+ 0.21 & 39.11+0.19 & 27.8 + 0.19 & 31.56+0.18 & 26.48 0.19  & 28.87+0.18 \\ 
IIC \cite{tao2020self} & No & No & 56.81+.23 & 78.74 + 0.19 & 34.66+ 0.22 & 49.57+ 0.23 & 37.73+0.22 & 51.1+0.22 \\ 
% PRP \cite{yao2020video} & 57.8 ± 3.0 & 80.2 ± 1.3 & 34.7 ± 9.20 & 54.0 ± 3.90 & - & - \\ \hline
Pace Prediction \cite{wang2020self} & No & No &  25.58+0.17 & 26.58+.16 & 26.21+17 & 27.09+0.16 & 22.42+0.17 & 22.94 +0.15 \\ 
MemDPC \cite{Han20} & No & No & 45.71+0.17 & 60.48+0.15 & 36.92+0.18 & 48.97+0.19 & 29.87+0.21 & 38.06+0.21 \\ 
CoCLR  \cite{Han20CoCLR} & No & No & 50.38+0.24 & 69.11+0.22 & 30.49+0.21 & 42.8+0.23 & 36.77+0.22 & 48.09+.24 \\ 

CVRL++ \cite{qian2020spatiotemporal} & No & No & 63.00 ± 0.21 & 87.8 ± 0.15 & 44.21 ± 0.23 & 60.35 ± 0.23 & 53.26 $\pm$ 0.24 & 71.39 $\pm$ 0.22\\ 
 \hline
% \methodname~(Ours) (3D stream only)  & No & No & 63.0 ±  &  87.8 ± 0.15  & 44.21 ± & 60.35 ±  0.23  & 53.26±0.24 & 71.39±0.22\\ 


\methodname~(ProtoNet~\cite{snell2017prototypical})  & No & No & 42.47 ± 0.42  & 72.58 ± 0.39  & 36.01 ± 0.40 & 48.25 ± 0.43   & 31.20 ± 0.39 & 55.96 ± 0.44\\ 
\methodname~(Baseline++~\cite{chen2018closer}) & No & No & 70.42 ± 0.45 & 89.08 ± 0.30 & 42.98 ± 0.47 & 61.83 ± 0.46 & 56.10 ± 0.47 & 73.37 ± 0.43 \\ 
\methodname~(Ours)  w/o Action  & No & No &  &  &   &   & 50.54 $\pm$ 0.23 & 65.59 $\pm$ 0.24 \\ 
\methodname~(Ours) w/o Appearance  & No & No &  &  &  &   & 53.26 $\pm$ 0.24 & 71.39 $\pm$ 0.22 \\ 
\methodname~(Ours) w/o $\mathcal{L}^{joint}_{NCE}$  & No & No &  & & &  & 58.59 $\pm$ 0.43 & 77.04 $\pm$ 0.39 \\ 
\methodname~(Ours)  & No & No & \textbf{73.41 ± 0.24}  & \textbf{91.29 ± 0.14} & \textbf{47.21 ± 0.23}  &  \textbf{65.28 ± 0.28} & \textbf{61.61 ± 0.46} & \textbf{79.20 ± 0.39} \\ 
\hline


\end{tabular}%
}
\caption{Few-shot video classification results. We report 5-way video classification accuracy on meta-testing set. Our approach surpasses previous supervised state-of-the-arts by a large margin.}
\label{tab:fsvar}

\end{table*}

==> tables/FSVAR_comb_bkp.tex <==
\begin{table*}[t]
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{|l|c|c|c|c|c|c|c|c|}
\hline
\multirow{2}{*}{Methods} & \multicolumn{2}{c|}{Supervision} & \multicolumn{2}{c|}{UCF101} & \multicolumn{2}{c|}{HMDB51} & \multicolumn{2}{c|}{Kinetics100} \\ \cline{2-9} 
 & \multicolumn{1}{l|}{Sup. Pretraining} & \multicolumn{1}{l|}{Base Sup.} & 1-shot & 5-shot & 1-shot & 5-shot & 1-shot & 5-shot \\ \hline
Matching Net \cite{zhu2018compound} & Imagenet-2D & Yes & - & - & - & - & 53.3 & 74.6 \\ 
MAML \cite{zhu2018compound} & Imagenet-2D & Yes & - & - & - & - & 54.2 & 75.3 \\ 
CMN \cite{zhu2018compound} & Imagenet-2D & Yes & - & - & - & - & 60.5 & 78.9 \\ 
TARN \cite{bishay2019tarn} & Sports-1M & Yes & - & - & - & - & 66.6 & 80.7 \\ 
OTAM \cite{Cao_2020_CVPR} & Imagenet-2D & Yes & - & - & - & - & 73.0 & 85.8 \\
R-3DFSV  \cite{xian2020generalized} & Sports-1M & Yes & - & - & - & - & 95.3 & 97.8 \\ 
ProtoGAN \cite{kumar2019protogan} & Sports-1M  & Yes  & 57.8  $\pm$  3.0 & 80.2  $\pm$  1.3 & 34.7  $\pm$  9.20 & 54.0  $\pm$  3.90 & - & - \\ 
AmeFu-Net \cite{fu2020depth} & Imagenet-2D & Yes & 85.1 & 95.5 & 60.2 & 75.5  & 74.1  & 86.8 \\ 
RVN \cite{cao2020few} & Kinetics-400 & Yes  & 88.71  $\pm$  0.19 & 96.78  $\pm$  0.08 & 63.43  $\pm$  0.28 & 79.69  $\pm$  0.20 & - & - \\ \hline
ARN  \cite{zhang2020few}  & No & Yes & 66.32  $\pm$  0.99 & 83.12  $\pm$  0.70 & 45.15  $\pm$  0.96 & 60.56  $\pm$  0.86 & 63.7 & 82.4 \\ \hline

3DRotNet \cite{jing2018self} & No & No & 38.43 $\pm$ 0.23	& 33.61 $\pm$ 0.15 & 27.35 $\pm$  0.2 & 26.84 $\pm$ 0.13 & 27.53 $\pm$  0.2 &	25.54 $\pm$ 0.13 \\ 
VCOP \cite{xu2019self}  & No & No & 32.91 $\pm$  0.21 & 39.11 $\pm$ 0.19 & 27.8  $\pm$  0.19 & 31.56 $\pm$ 0.18 & 26.48 0.19  & 28.87 $\pm$ 0.18 \\ 
IIC \cite{tao2020self} & No & No & 56.81 $\pm$ .23 & 78.74  $\pm$  0.19 & 34.66 $\pm$  0.22 & 49.57 $\pm$  0.23 & 37.73 $\pm$ 0.22 & 51.1 $\pm$ 0.22 \\ 
% PRP \cite{yao2020video} & 57.8  $\pm$  3.0 & 80.2  $\pm$  1.3 & 34.7  $\pm$  9.20 & 54.0  $\pm$  3.90 & - & - \\ \hline
Pace Prediction \cite{wang2020self} & No & No &  25.58 $\pm$ 0.17 & 26.58 $\pm$ .16 & 26.21 $\pm$ 17 & 27.09 $\pm$ 0.16 & 22.42 $\pm$ 0.17 & 22.94  $\pm$ 0.15 \\ 
MemDPC \cite{Han20} & No & No & 45.71 $\pm$ 0.17 & 60.48 $\pm$ 0.15 & 36.92 $\pm$ 0.18 & 48.97 $\pm$ 0.19 & 29.87 $\pm$ 0.21 & 38.06 $\pm$ 0.21 \\ 
CoCLR  \cite{Han20CoCLR} & No & No & 51.99 $\pm$ 0.46 & 72.17 $\pm$ 0.42 & 30.49 $\pm$ 0.21 & 42.8 $\pm$ 0.23 & 36.77 $\pm$ 0.22 & 48.09 $\pm$ .24 \\ 

CVRL \cite{qian2020spatiotemporal} & No & No & 63.0  $\pm$  0.21 & 87.8  $\pm$  0.15 & 44.21  $\pm$  0.23 & 60.35  $\pm$  0.23 & 53.26  $\pm$  0.24 & 71.39  $\pm$  0.22\\ 
 \hline
% \methodname~(Ours) (3D stream only)  & No & No & 63.0  $\pm$   &  87.8  $\pm$  0.15  & 44.21  $\pm$  & 60.35  $\pm$   0.23  & 53.26 $\pm$ 0.24 & 71.39 $\pm$ 0.22\\ 


\methodname~(ProtoNet~\cite{snell2017prototypical})  & No & No & 42.47  $\pm$  0.42  & 72.58  $\pm$  0.39  & 36.01  $\pm$  0.40 & 48.25  $\pm$  0.43   & 31.20  $\pm$  0.39 & 55.96  $\pm$  0.44\\ 
\methodname~(Baseline $\pm$  $\pm$ ~\cite{chen2018closer}) & No & No & 70.42  $\pm$  0.45 & 89.08  $\pm$  0.30 & 42.98  $\pm$  0.47 & 61.83  $\pm$  0.46 & 56.10  $\pm$  0.47 & 73.37  $\pm$  0.43 \\ 

\methodname~(Ours)  & No & No & \textbf{75.70  $\pm$  0.42}  & \textbf{92.50  $\pm$  0.24} & \textbf{47.44  $\pm$  0.44}  &  \textbf{66.13  $\pm$  0.33} & \textbf{61.61  $\pm$  0.46} & \textbf{79.20  $\pm$  0.39} \\ 
\hline


\end{tabular}%
}
\caption{Few-shot video classification results. We report 5-way video classification accuracy on the meta-testing set. Our approach surpasses previous supervised state-of-the-arts by a large margin.}
\label{tab:fsvar}

\end{table*}

==> tables/FSVAR_combined.tex <==
\begin{table*}[t]
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{|l|c|c|c|c|c|c|c|c|}
\hline
\multirow{2}{*}{Methods} & \multicolumn{2}{c|}{Supervision} & \multicolumn{2}{c|}{UCF101} & \multicolumn{2}{c|}{HMDB51} & \multicolumn{2}{c|}{Kinetics100} \\ \cline{2-9} 
 & \multicolumn{1}{l|}{Pretraining} & \multicolumn{1}{l|}{Base Class} & 1-shot & 5-shot & 1-shot & 5-shot & 1-shot & 5-shot \\ \hline
Matching Net \cite{zhu2018compound} & Imagenet-2D & Yes & - & - & - & - & 53.3 & 74.6 \\ 
MAML \cite{zhu2018compound} & Imagenet-2D & Yes & - & - & - & - & 54.2 & 75.3 \\ 
CMN \cite{zhu2018compound} & Imagenet-2D & Yes & - & - & - & - & 60.5 & 78.9 \\ 
TARN \cite{bishay2019tarn} & Sports-1M & Yes & - & - & - & - & 66.6 & 80.7 \\ 
OTAM \cite{Cao_2020_CVPR} & Imagenet-2D & Yes & - & - & - & - & 73.0 & 85.8 \\
R-3DFSV  \cite{xian2020generalized} & Sports-1M & Yes & - & - & - & - & \textcolor{blue}{95.3} & \textcolor{blue}{97.8} \\ 
ProtoGAN \cite{kumar2019protogan} & Sports-1M  & Yes  & 57.8  $\pm$  3.0 & 80.2  $\pm$  1.3 & 34.7  $\pm$  9.20 & 54.0  $\pm$  3.90 & - & - \\ 
AmeFu-Net \cite{fu2020depth} & Imagenet-2D & Yes & 85.1 & 95.5 & 60.2 & 75.5  & 74.1  & 86.8 \\ 
RVN \cite{cao2020few} & Kinetics-400 & Yes  & \textcolor{blue}{88.71  $\pm$  0.19} & \textcolor{blue}{96.78  $\pm$  0.08} & \textcolor{blue}{63.43  $\pm$  0.28} & \textcolor{blue}{79.69  $\pm$  0.20} & - & - \\ \hline
ARN  \cite{zhang2020few}  & No & Yes & 66.32  $\pm$  0.99 & 83.12  $\pm$  0.70 & 45.15  $\pm$  0.96 & 60.56  $\pm$  0.86 & 63.7 & 82.4 \\ \hline

3DRotNet \cite{jing2018self} & No & No & 39.43 $\pm$ 0.48	& 33.61 $\pm$ 0.34 & 32.35 $\pm$  0.42 & 27.84 $\pm$ 0.40 & 27.53 $\pm$  0.36 &	25.54 $\pm$ 0.39 \\ 
VCOP \cite{xu2019self}  & No & No & 32.91 $\pm$  0.42 & 39.11 $\pm$ 0.37 & 27.8  $\pm$  0.37 & 31.56 $\pm$ 0.35 & 26.48 $\pm$ 0.37  & 28.87 $\pm$ 0.36 \\ 
IIC \cite{tao2020self} & No & No & 56.81 $\pm$ 0.46 & 78.74  $\pm$  0.37 & 34.66 $\pm$  0.41 & 49.57 $\pm$  0.44 & 37.73 $\pm$ 0.43 & 51.11 $\pm$ 0.43 \\ 
% PRP \cite{yao2020video} & 57.8  $\pm$  3.0 & 80.2  $\pm$  1.3 & 34.7  $\pm$  9.20 & 54.0  $\pm$  3.90 & - & - \\ \hline
Pace Prediction \cite{wang2020self} & No & No &  25.58 $\pm$ 0.33 & 26.58 $\pm$ 0.31 & 26.21 $\pm$ 0.33 & 27.09 $\pm$ 0.31 & 22.42 $\pm$ 0.33 & 22.94  $\pm$ 0.30 \\ 
MemDPC \cite{Han20} & No & No & 49.27 $\pm$ 0.44 & 67.38 $\pm$ 0.45 & 30.33 $\pm$ 0.40 & 41.15 $\pm$ 0.42 & 42.01 $\pm$ 0.41 & 53.90 $\pm$ 0.43 \\ 
CoCLR  \cite{Han20CoCLR} & No & No & 51.99 $\pm$ 0.46 & 72.17 $\pm$ 0.42 & 31.29 $\pm$ 0.40 & 44.92 $\pm$ 0.45 & 37.59 $\pm$ 0.42 & 51.11 $\pm$ 0.43 \\ 

CVRL \cite{qian2020spatiotemporal} & No & No & 63.00  $\pm$  0.41 & 87.8  $\pm$  0.30 & 44.21  $\pm$  0.45 & 60.35  $\pm$  0.45 & 53.26  $\pm$  0.48 & 71.39  $\pm$  0.44\\ 
 \hline
% \methodname~(Ours) (3D stream only)  & No & No & 63.0  $\pm$   &  87.8  $\pm$  0.15  & 44.21  $\pm$  & 60.35  $\pm$   0.23  & 53.26 $\pm$ 0.24 & 71.39 $\pm$ 0.22\\ 


\methodname~(ProtoNet~\cite{snell2017prototypical})  & No & No & 42.47  $\pm$  0.42  & 72.58  $\pm$  0.39  & 36.01  $\pm$  0.40 & 48.25  $\pm$  0.43   & 31.20  $\pm$  0.39 & 55.96  $\pm$  0.44\\ 
\methodname~(Baseline ++ ~\cite{chen2018closer}) & No & No & 70.42  $\pm$  0.45 & 89.08  $\pm$  0.30 & 42.98  $\pm$  0.47 & 61.83  $\pm$  0.46 & 56.10  $\pm$  0.47 & 73.37  $\pm$  0.43 \\ 

\methodname~(Ours)  & No & No & \textbf{76.38 $\pm$ 0.40}  & \textbf{92.50 $\pm$ 0.24} & \textbf{47.55 $\pm$ 0.45}  &  \textbf{66.13 $\pm$ 0.33} & \textbf{62.80 $\pm$ 0.45} & \textbf{79.55 $\pm$ 0.39} \\ 
\hline


\end{tabular}%
}
% \caption{Few-shot video classification results. We report 5-way video classification accuracy on the meta-testing set. Our approach surpasses previous supervised state-of-the-arts by a large margin.}
\caption{Results on UCF101, HMDB51 and Kinetics100 dataset for 5-way, 1-shot and 5-shot few-shot action recogniton. Our method \methodname~is able to outperform existing SoTA approaches on video-based self-supervision by large margins on the few-shot benchmark. It also performs competitively \wrt supervised few-shot approaches. On UCF101 and HMDB51, \methodname~is able to outperform ARN that uses only base class supervision. Values in \textcolor{blue}{blue} represent SoTA across all levels of supervision.}
\label{tab:fsvar}

\end{table*}

==> tables/LRablation.tex <==
\begin{table}[h]
\resizebox{\columnwidth}{!}{%
\begin{tabular}{|c|cccccc|}
\hline
\diagbox{steps}{LR}
 & 0.001 & 0.01 & 0.1 & 10 & 50 & 100 \\ \hline
10 &  &  &  &  &  &  \\
50 &  &  &  &  &  &  \\
100 &  &  &  &  &  &  \\
500 &  &  &  &  &  &  \\ \hline
\end{tabular}
}
\caption{Meta-testing Learning rate comparasion}
\label{tab:LRtable}
\end{table}

==> tables/SS.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage{graphicx}
\begin{table*}[t]
 \footnotesize
\centering
% \resizebox{\textwidth}{!}{%
\begin{tabular}{|l|c|c|c|c|c|c|}
\hline
\multirow{2}{*}{Methods} & \multicolumn{2}{c|}{UCF101} & \multicolumn{2}{c|}{HMDB51} & \multicolumn{2}{c|}{Kinetics100} \\ \cline{2-7} 
 & 1-shot & 5-shot & 1-shot & 5-shot & 1-shot & 5-shot \\ \hline
3DRotNet \cite{jing2018self} & 38.43+0.23	& 33.61+0.15 & 27.35+ 0.2 & 26.84+0.13 & 27.53+ 0.2 &	25.54+0.13 \\ \hline
VCOP \cite{xu2019self}  & 32.91+ 0.21 & 39.11+0.19 & 27.8 + 0.19 & 31.56+0.18 & 26.48 0.19  & 28.87+0.18 \\ \hline
IIC \cite{tao2020self} & 56.81+.23 & 78.74 + 0.19 & 34.66+ 0.22 & 49.57+ 0.23 & 37.73+0.22 & 51.1+0.22 \\ \hline
% PRP \cite{yao2020video} & 57.8 ± 3.0 & 80.2 ± 1.3 & 34.7 ± 9.20 & 54.0 ± 3.90 & - & - \\ \hline
Pace Prediction \cite{wang2020self} &  25.58+0.17 & 26.58+.16 & 26.21+17 & 27.09+0.16 & 22.42+0.17 & 22.94 +0.15 \\ \hline
MemDPC \cite{Han20} & 45.71+0.17 & 60.48+0.15 & 36.92+0.18 & - & 29.87+0.21 & 38.06+0.21 \\ \hline
CoCLR  \cite{Han20CoCLR} & 50.38+0.24 & 69.11+0.22 & 30.49+0.21 & 42.8+0.23 & 36.77+0.22 & 48.09+.24 \\ \hline

CVRL++ \cite{qian2020spatiotemporal} & 63.0 ± 0.21 & 87.8 ± 0.15 & 44.21 ± 0.23 & 60.35 ± 0.23 & 53.26 $\pm$ 0.24 & 71.39 $\pm$ 0.22\\ \hline
% CVRL  \cite{qian2020spatiotemporal} & 44.21 & tba & 67.31 & tba & 55.4 & tba \\ 
\methodname~(Ours) & \textbf{73.41 ±}  & \textbf{91.29 ± 0.14} & \textbf{47.21 ±}  &  \textbf{65.28 ± 0.28} & \textbf{61.61 ± 0.46} & \textbf{79.20 ± 0.39} \\ \hline
% Ours VideoCLR Ablation2 & 47.21 & tba & 73.41 & tba & 59.97 & tba \\ \hline
% Ours VideoCLR Ablation3 & 47.21 & tba & 73.41 & tba & 59.97 & tba \\ \hline
% \rowcolor{lightgray}
% Supervised Baseline & 47.21 & tba & 73.41 & tba & 59.97 & tba \\ \hline
\end{tabular}%
% }
\caption{Comparision of Video Self-Supervised Techniques for the Few-shot Action Recogntion Task.}
\label{tab:SS}
\end{table*}

==> tables/ablations.tex <==

% \begin{table}[h]
% \resizebox{\columnwidth}{!}{%
% \begin{tabular}{cccc|cc}
% \hline
% \multicolumn{1}{l}{ 2D Stream} & 3D Stream & MM-NCE & Multi-scale & 1-shot & 5-shot \\ \hline
% \checkmark \par &  &  &  & 50.54 $\pm$ 0.23 & 65.59 $\pm$ 0.24 \\
%  & \checkmark \par &  &  & 53.26 $\pm$ 0.24 & 71.39 $\pm$ 0.22 \\
% \checkmark \par & \checkmark \par &  &  & 53.26 $\pm$ 0.24 & 71.39 $\pm$ 0.22 \\
% \checkmark \par & \checkmark \par & \checkmark \par &  & 58.96 $\pm$ 0.78 & 77.62 $\pm$ 0.31 \\
% \checkmark \par & \checkmark \par & \checkmark \par & \checkmark \par & 61.61 $\pm$ 0.46  & 79.20 $\pm$ 0.39 \\ \hline
% \end{tabular}
% }
% \caption{Ablations of different modules of \methodname~ on the Kinetics100  }
% \label{tab:ablation}
% \end{table}



% \begin{table}[h]
% \resizebox{\columnwidth}{!}{%
% \begin{tabular}{cccc|cc}
% \hline
% \multicolumn{1}{l}{ 2D Stream} & 3D Stream & MM-NCE & 1-shot & 5-shot \\ \hline
% \checkmark \par &  &   & 50.54 $\pm$ 0.23 & 65.59 $\pm$ 0.24 \\
%  & \checkmark \par &   & 53.26 $\pm$ 0.24 & 71.39 $\pm$ 0.22 \\
% \checkmark \par & \checkmark \par &   & 58.59 $\pm$ 0.43 & 77.04 $\pm$ 0.39 \\
% \checkmark \par & \checkmark \par &  \checkmark \par & 61.61 $\pm$ 0.46  & 79.20 $\pm$ 0.39 \\ \hline
% \end{tabular}
% }
% \caption{Ablations of different modules of \methodname~ on the Kinetics100  }
% \label{tab:ablation}
% \end{table}


% \begin{table}[h]
% \resizebox{\columnwidth}{!}{%
% \begin{tabular}{l|cc}
% \hline
% Method & 1-shot & 5-shot \\ \hline
% \methodname~(ours) w/o Action & 50.54 $\pm$ 0.23 & 65.59 $\pm$ 0.24 \\
% \methodname~(ours) w/o Appearance & 53.26 $\pm$ 0.24 & 71.39 $\pm$ 0.22 \\
% \methodname~(ours) w/o $\mathcal{L}^{joint}_{NCE}$ & 58.59 $\pm$ 0.43 & 77.04 $\pm$ 0.39 \\
% \methodname~(ours)& 61.61 $\pm$ 0.46  & 79.20 $\pm$ 0.39 \\ \hline
% \end{tabular}
% }
% \caption{Ablation study of \methodname~ on Kinetics100 1 and 5-shot, 5-way}
% \label{tab:ablation}
% \end{table}


\begin{table*}[t]
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{|l|c|c|c|c|c|c|c|c|}
\hline
\multirow{2}{*}{Methods} & \multicolumn{2}{c|}{Supervision} & \multicolumn{2}{c|}{UCF101} & \multicolumn{2}{c|}{HMDB51} & \multicolumn{2}{c|}{Kinetics100} \\ \cline{2-9} 
 & \multicolumn{1}{l|}{Pretraining} & \multicolumn{1}{l|}{Base Class} & 1-shot & 5-shot & 1-shot & 5-shot & 1-shot & 5-shot \\ \hline

\methodname~(Ours)  w/o Action  & No & No & 65.26 $\pm$ 0.46 & 83.26 $\pm$ 0.36 & 37.92 $\pm$ 0.46   & 50.2 $\pm$ 0.44  & 50.54 $\pm$ 0.23 & 65.59 $\pm$ 0.48 \\ 
\methodname~(Ours) w/o Appearance  & No & No & 63.00  $\pm$  0.41 & 87.8  $\pm$  0.30 & 44.21  $\pm$  0.45 & 60.35  $\pm$  0.45 & 53.26  $\pm$  0.48 & 71.39  $\pm$  0.44 \\ 
\methodname~(Ours) w/o Hard Episodes  & No & No & 73.83 $\pm$ 0.42 & 91.44 $\pm$ 0.26 & 45.31 $\pm$ 0.46 & 64.57 $\pm$ 0.41 & 58.59 $\pm$ 0.43 & 77.04 $\pm$ 0.39 \\ 
\methodname~(Ours)  & No & No & \textbf{75.70 $\pm$ 0.42}  & \textbf{92.50 $\pm$ 0.24} & \textbf{47.44 $\pm$ 0.44}  &  \textbf{66.13 $\pm$ 0.33} & \textbf{61.61 $\pm$ 0.46} & \textbf{79.20 $\pm$ 0.39} \\ 
\hline


\end{tabular}%
}
\caption{Ablation study of \methodname~highlighting the impact of two-stream architecture and MM-NCE loss on few-shot performance.}
\label{tab:ablation}

\end{table*}
% \vspace{-5em}

==> tables/mixed_data.tex <==
\begin{table}[h]
% \resizebox{\columnwidth}{!}{%
\centering
\small
\begin{tabular}{l|cc}
\hline
Method & 1-shot & 5-shot \\ \hline
CVRL \cite{qian2020spatiotemporal} & 60.47  $\pm$ 0.23 & 80.81 $\pm$ 0.19 \\
\methodname~(ours)& \textbf{68.12  $\pm$ 0.44}  & \textbf{85.96 $\pm$ 0.33}\\ \hline
\end{tabular}
% }
\caption{Mixed-dataset performance on 5-shot, 1-way and 5-way}
\label{tab:mixed}
\end{table}
